Gillian: Compositional Symbolic Execution for All

We present Gillian, a language-independent framework for the development of compositional symbolic analysis tools. Gillian supports three flavours of analysis: whole-program symbolic testing, full verification, and bi-abduction. It comes with fully parametric meta-theoretical results and a modular implementation, designed to minimise the instantiation effort required of the user. We evaluate Gillian by instantiating it to JavaScript and C, and perform its analyses on a set of data-structure libraries, obtaining results that indicate that Gillian is robust enough to reason about real-world programming languages.

==> sections/sem_martin.tex <==
%!TEX root = ../main.tex
\section{Parametric Symbolic Execution}
\label{sec:sem}

\subsection{Syntax and Semantics}

\gil is a parameterisable goto language with top-level procedures.
\mbinline{Parameterisable by what? I would say something like this:
    \gil (pronounced \textipa{/\t{dZ}il/}) is a goto language with top-level procedures.
    It is parameterised by a set of actions… etc.}
A \gil program can be viewed as a set of top-level procedures with distinct names.
\mbinline{“can be viewed”: it’s not clear whether this is a formal or informal sentence.
    What about saying that a \gil program is composed of top-level procedures, each with a distinct name.
    I guess that one of these procedures is the main one and is associated a special name?}
Every \gil program is parameterised by a set $\actions$ of actions for acting on a given \gil state.
\mbinline{Is this the \gil programming language or the \gil programs that are parameterised?
    I think that it is the \gil program.}
\mbinline{From what I understand, what you call “\gil state” is something that looks like the heap
    (but as it is defined by the user, we have no control over what it might look like, which is cool),
    but does not include the \gil environment.
    If so, it is not clear in this first sentence.}
\polish{Say something about \gil states being opaque and awesome.}

%\myparagraph{Syntax} The syntax of \gil is given below. 
%
\medskip
\begin{display}{The Syntax of \gil}
\begin{tabular}{ll}
   $\vl \in \vals$ $\defeq$ $\num \in \nums \mid i \in \ints \mid \str \in \strs \mid \bool \in \bools \mid \loc \in \locs \mid \type \in \types \mid \fid \in \fids \mid \lst{\vl}$ 
   & 
   $\e \in \exprs$ $\defeq$ $\vl \mid \x \in \xs \mid \unop{\e} \mid \binop{\e_1}{\e_2}$
   %  \lx  \in \lxs
   \\[3pt]
   % 
    \multicolumn{2}{l}{$\cm \in \cmds{\actions}$ $\defeq$ $\x := \e \mid  \x := \act(\e) \mid \ifgoto{\e}{i} \mid \e(\e') 
                                     \mid  \return{\e} \mid \x := \fresh{j} \mid \x := \symb{j} \mid  \fail{e} \mid \vanish $}
    %
    \\[3pt]
    $\proc \in \procs{\actions}$ $\defeq$ $\procedure{f}{\x}{\lst{\cm}}$
    & 
    $\prog \in \progs{\actions}$ $:$ $\fids \pmap \procs{\actions}$
 \end{tabular}
\end{display}
\mbinline{I understand that you are trying to save space,
    but the definition of \(e\) has to be in its own line.
    It took me far too much time to notice that it was defined 1em after the values.}
\mbinline{Only now I realised that \(\proc\) and \(\prog\) have different fonts.
    This should be emphased more, either by saying “Notice the difference of fonts between serif~\(\proc\)
    and sans serif~\(\prog\), or by adding an underline or a diacritic to one of these.}
\mbinline{
    I would have written
    “$\prog \in \progs{\actions} = \fids \pmap \procs{\actions}$”
    instead of “$\prog \in \progs{\actions}$ $:$ $\fids \pmap \procs{\actions}$”.
    Also, recall that \(f \in \fids\) in the same line than the definition of procedures.}
%
\gil \emph{values}, $\vl \in \vals$, include numbers, integers, strings, booleans,  locations, types, procedure identifiers, and lists of values.
\mbinline{Wait, types are values? This needs clarification: what kind of types are we talking about here?}
\gil~\emph{expressions}, $\e \in \exprs$, include values, program variables $\x$, and various unary and binary operators. %Symbolic variables 

\gil \emph{commands} include: variable assignments; actions
\mbinline{Inserts \(\act \in \actions\) here.}
for operating on the given state;
conditional gotos;  procedure calls; a $\kwT{return}$
\mbinline{(Nitpicking) the kwT command inserts an additional space. It feels strange.}
command for terminating the execution of 
the current procedure; a distinguished command $\kwT{fresh}$ for generating fresh locations; 
a distinguished command $\kwT{symb}$ for generating \polish{arbitrary} values; 
a command $\kwT{fail}$ for terminating the execution of the entire program with an error; 
and, finally, a command $\vanish$ for \emph{dropping} the current execution (e.g.\@ meaning that 
it terminates silently without generating a result).

The variable assignment, goto, return, fail, and vanish commands are straightforward. 
The procedure call is dynamic: the procedure identifier is obtained by evaluating the caller expression.
The commands $\kwT{fresh}$ and $\kwT{symb}$ are annotated with a unique identifier $j$ to be used 
by the semantics. 
Finally, the action command $\x := \act(\e)$ executes the action $\act \in \actions$ on the 
current state with the argument resulting from the evaluation of $\e$. 

A \gil procedure is of the form $\procedure{f}{\x}{\lst{\cm}}$, where $\f$ is its identifier, $\x$ is its formal parameter, 
and its body $\lst{\cm}$  is a sequence of \gil commands. 
In order not to clutter the formalism, we assume that procedures have a single parameter. 
In the implementation, however, procedures are allowed to have multiple parameters. 
%
A \gil program $\prog \in \progs{\actions}$ is a partial function mapping procedure identifiers 
to their corresponding procedures. 

\myparagraph{Semantics} 
The semantics of \gil is parameterised by a state module $\gstate \in \gstates$.
A state module describes: 
\etag{1} the set $\sset{\gstate}$ of states on which the given \gil program is going to operate;  
\etag{2} the set $\gval$ of values stored in those states; and 
\etag{3} the \emph{actions} $\act \in \actions$ that can be performed on those states. 
In particular, every state module defines a function 
$\kwT{ea} : \actions \tmap \sset{\gstate} \tmap \gval \pmap \power{\sset{\gstate} \times \gval}$, 
written $\kwT{ea}(\act, \st, \gv)$, for executing the action $\act$ on the state $\st$
with argument $\gv$. Actions can have multiple results, each consisting of new state $\st'$
and a return value $\gv'$.  
Hence, the semantics of \gil is \emph{potentially} non-deterministic. 
Observe, however, that one can always instantiate the semantics of \gil with a state module 
whose actions are all deterministic, obtaining a deterministic semantics. 

\vspace{-10pt}\mbinline{This negative space is far too big.  I could notice that something was wrong with the space and realised that you have placed this negative space afterwards.  If you really want to place a negative space, remove 3pt before the itemize below and only remove 5pt here.}
\begin{definition}[State Module]\label{def:state:module}
A state module $\gstate \in \gstates$ is a triple $\tup{\sset{\gstate}, \gval, \actions}$ consisting of: 
\etag{1} a set of states $\sset{\gstate}$, \etag{2} a set of values $\gval$, and \etag{3} a set of 
actions $\actions$. A state module additionally defines the following functions for acting on states: 

\begin{itemize}
   \item $\kwT{setVar} : \sset{\gstate} \tmap \xs \tmap \gval \tmap \sset{\gstate}$ 
            \hfill (\emph{notation:} $\kwT{setVar}(\st, \x, \vl) \equiv \st.\kwT{setVar}(\x, \vl)$) 
   %
   \item $\kwT{setStore} : \sset{\gstate} \tmap (\xs \pmap \gval) \tmap \sset{\gstate}$ 
            \hfill (\emph{notation:} $\kwT{setStore}(\st, \sto) \equiv \st.\kwT{setStore}(\sto)$) 
   %
   \item $\kwT{store} : \sset{\gstate} \tmap \sset{\gstate}$ 
            \hfill (\emph{notation:} $\kwT{store}(\st) \equiv \st.\kwT{store}$) 
   %
   \item $\kwT{ee} : \sset{\gstate} \tmap \exprs \pmap \gval$ 
            \hfill (\emph{notation:} $\kwT{ee}(\st, \e) \equiv \st.\kwT{ee}(\e)$) 
   %
   \item $\kwT{ea} : \actions \tmap \sset{\gstate} \tmap \gval \pmap \power{\sset{\gstate} \times \gval}$ 
            \hfill (\emph{notation:} $(\st', \vl') \in \kwT{ea}(\act, \st, \vl) \equiv \action{\st}{\act}{v}{(\st', v')}$) 
\end{itemize}
\end{definition}

\mbinline{At this stage of the paper, I still don’t know what is the difference between \(\vals\) and \(\gval\).
    I guess that \(\gval\) are the values stored in the \gil environment
    and that \(\vals\) are the one stored in the state.
    I guess that there can be some linked between these,
    but by double-checking with the definition above, it seems that \(\gval\)
    is a constructor of \(\vals\).
    There should be an intuition about what is \(\gval\) at this point
    (or even better, in the paragraph before the definition).}

A state module $\gstate =  \tup{\sset{\gstate}, \gval, \actions}$ is said to be \emph{proper} 
if and only if it defines the following three distinguished actions: $\kwT{assume}$,
 $\kwT{fresh}$, and  $\kwT{symb}$ (i.e. $\set{\kwT{assume}, \kwT{fresh}, \kwT{symb}} \subseteq A$).
 In the following, we use $\actionsZ$  to refer to the set $\set{\kwT{assume}, \kwT{fresh}, \kwT{symb}}$.

As the variable store is kept as part of the state, \gil state modules are expected to define 
the following functions for interacting with the variable store: 
\etag{1} $\kwT{setVar}(\st, \x, \vl)$ for setting $\x$ to $\vl$ in the variable store of $\st$;
\etag{2} $\kwT{setStore}(\st, \x, \sto)$ for replacing the store of $\st$ with $\sto$; 
\etag{3} $\kwT{store}(\st)$ for obtaining the store of $\st$ \mbinline{I don’t understand the type of \(\kwT{store}\): is it more than an identity function?}; and 
\etag{4} $\kwT{ee}(\st, \e)$ for evaluating the expression $\e$ in the store of $\st$. 
\polish{Why did we put the store inside the state?}
Finally, Definition~\ref{def:state:module} formalises the notion of state module. 

\begin{figure}[!t]
{\footnotesize
\begin{mathpar}
\inferrule[\textsc{Assignment}]
  {
    \cmd(\prog, \cs, i) = \x := \e
    \and
    \ee{\st}{\e} = v
    %\\\\
    %\actionT{\st}{setVar}{\x, v}{\st'}
  }{\semtrans{\st, \cs, i}{\st.\kwT{setVar}(\x, v), \cs, i{+}1}{}{\prog}{}}  	 
 %
 \and
 %
\inferrule[\textsc{Action}]
  {
    \cmd(\prog, \cs, i) = \x := \act(\e)
    \and
    \ee{\st}{\e} = v
    \\\\
     \action{\st}{\act}{v}{(\st', v')}
     %\and
    %\actionT{\st'}{setVar}{\x, v'}{\st''}
  }{\semtrans{\st, \cs, i}{\st'.\kwT{setVar}(\x, v'), \cs, i{+}1}{}{\prog}{}}  	 
\\
%
\inferrule[\textsc{IfGoto - True}]
  {
    \cmd(\prog, \cs, i) = \ifgoto{\e}{i}
    \and
    \ee{\st}{\e} = v
    \\\\
    \actionT{\st}{assume}{v}{\st'}
  }{\semtrans{\st, \cs, i}{\st', \cs, j}{}{\prog}{}}  	 
%
\and
%
\inferrule[\textsc{IfGoto - False}]
  {
    \cmd(\prog, \cs, i) = \ifgoto{\e}{i}
    \and
    \ee{\st}{\e} = v
    \\\\
    \actionT{\st}{assume}{v}{\st'}
  }{\semtrans{\st, \cs, i}{\st', \cs, j}{}{\prog}{}}  	 
%
\\
%
\inferrule[\textsc{Fresh}]
  {
      \cmd(\prog, \cs, i) = \x := \fresh{j}
      \and
      \ee{\st}{\e} = v
      \\\\ 
      \actionT{\st}{fresh}{v}{(\st', v')}
  }{
    \semtrans{\st, \cs, i}{\st'.\kwT{setVar}(\x, v'), \cs, i{+}1}{}{\prog}{}
  }
 %
 \and 
 %
 \inferrule[\textsc{Symb}]
  {
     \cmd(\prog, \cs, i) = \x := \symb{j}
      \and 
      \ee{\st}{\e} = v
      \\\\ 
    \actionT{\st}{symb}{v}{(\st', v')}
  }{
    \semtrans{\st, \cs, i}{\st'.\kwT{setVar}(\x, v'), \cs, i{+}1}{}{\prog}{}
  }
  \\
%
\inferrule[\textsc{Call}]
  {
    \cmd(\prog, \cs, i) = \e(\e')
    \and
    \ee{\st}{\e} = \f
    \\\\
    \ee{\st}{\e'} = v
    \and
    \cs' = \vtup{\f, \x, \st.\kwT{store}, i+1} \cons \cs
    %\quad
    %\actionT{\st}{setStore}{\bconf{\f.\kwT{arg} \mapsto v}}{\st'}
  }{\semtrans{\st, \cs, i}{\st.\kwT{setStore}(\btup{\f.\kwT{arg} \mapsto v}), \cs', 0}{}{\prog}{}}  	
%
\and
%
\inferrule[\textsc{Return}]
  {
     \cmd(\prog, \cs, i) = \return{\e}
      \and
    \ee{\st}{\e} = v   
     \\\\
    \cs = \vtup{-, \x, \sto, j} \cons \cs'
    \and 
    \st' = \st.\kwT{setStore}(\sto)
  }{
    \semtrans{\st, \cs, i}{\st'.\kwT{setVar}(\x, v'), \cs', j}{}{\prog}{}
  }
  \\
  %
 \inferrule[\textsc{Top Return}]
  {
     \cmd(\prog, \cs, i) = \return{\e}
      \and
    \ee{\st}{e} = v
  }{
    \semtrans{\st, \vtup{\fid}, i}{\st, \cs, i}{}{\prog}{\normal{v}}
  } 
  %
  \and
  %
 \inferrule[\textsc{Fail}]
  {
     \cmd(\prog, \cs, i) = \fail{e}
      \and
    \ee{\st}{\e} = \vl
  }{
    \semtrans{\st, \cs, i}{\st, \cs, i}{}{\prog}{\error{\vl}}
  } 
\end{mathpar}}
%
\caption{Semantics of \gil: $\fullsemtrans{\st, \cs, i}{\st', \cs', j}{}{\prog}{\outcome'}{\outcome}$}
\label{fig:sem}
\vspace{-10pt}
%
\end{figure}

The semantics of \gil is defined in Figure~\ref{fig:sem} in small-step style. 
The small-step style means that the semantics must keep track of the execution 
context of the calling procedure every time a new procedure is called (so that it
knows where to return the control when the execution of the latter procedure is finished). 
To this end, we make use of call stacks~\polish{\cite{??}}. 
A \emph{call stack} $\cs$ is a \emph{non-empty} list of stack frames. 
A top level stack frame $\vtup{\f}$ consists solely of the identifier of the procedure which started the 
execution. 
An inner stack frame $\vtup{\f, \x, \sto, i}$ is composed of: 
\etag{1} the identifier $\f$ of the procedure being executed;
\etag{2} the variable $\x$ to which the return value of $\f$ will be assigned; 
\etag{3} the store $\sto$ of the caller of $\f$; and 
\etag{4} the index $i$ to which the control is transferred when the execution of $\f$ terminates.
\mbinline{I have no idea what \(i\) is at this stage of the paper: is this some kind of program point?
    (Note that it becomes clear later.  I would mention “program point” as some of intuition here anyway.)}

\medskip
\begin{display}{\gil Semantic Domains for $\gstate =  \tup{\sset{\gstate}, \gval, \actions}$}
\begin{tabular}{llll}
   %
   $\cs \in \css{\gstate} $ & $\defeq$ & $ \vtup{\f} \mid \vtup{\f, \x, \sto, i} \cons \cs$ & where: $\f \in \fids$, $\x \in \xs$, $\sto : \xs \pmap \gval$, $i \in \ints$\\
   %
   $\cf \in \cfs{\gstate}$    & $\defeq$ & $\tup{\prog, \st, \cs, i}$     & where: $\prog \in \progs{\actions}$, $\st \in \sset{\gstate}$, $\cs \in \css{\gstate}$, $i \in \ints$ \\
   % 
   $\outcome \in \outcomes$  & $\defeq$ &  $\cont \mid \normal{v} \mid \error{v}$ & where: $v \in \gval$
 \end{tabular}
\end{display}
\mbinline{There are three “|” symbols one after the other with very different meanings.
    Suggestion: play with the “left.” and “right.” commands to make the “mid” larger.
    You might have to do this in the other grammar definitions.
    Another solution is to redefine “mid” to increate the space it introduces.}
\mbinline{What is \(\css{}\)? I haven’t seen it defined. Also, mind its kerning.}

Semantic transitions for \gil commands have the form $\fullsemtrans{\st, \cs, i}{\st', \cs', j}{\gstate}{\prog}{\outcome'}{\outcome}$, 
meaning that, given a \gil program $\prog$, and starting from the state~$\st$, the evaluation of 
the $i$-th command of the leading procedure of the call stack $\cs$ generates the state~$\st'$ and  
the call stack~$\cs'$,  and the next command to be evaluated is the $j$-th command of the leading procedure 
of~$\cs'$. Observe that the semantic transition additionally consumes the \emph{outcome} of the previously 
executed command, $\outcome$, and generates a new outcome $\outcome'$. 
\gil has three possible outcomes: 
\etag{1} the continuation outcome, $\cont$, signifying that the execution should 
proceed; 
\etag{2} the return outcome $\normal{\gvl}$, signifying that there was a top level return with value $\gvl$; 
and 
\etag{3} the error outcome $\error{\gvl}$, signifying that the execution \emph{failed} with value $\gvl$. 
In the rules, the absence of an explicit outcome annotating a configuration is to be interpreted as the continuation outcome 
(e.g. we write $\fullsemtrans{\st, \cs, i}{\st', \cs', j}{\gstate}{\prog}{}{}$ to mean 
$\fullsemtrans{\st, \cs, i}{\st', \cs', j}{\gstate}{\prog}{\cont}{\cont}$). Naturally, 
a semantic transition can only occur when the outcome of the previous command is the continuation 
outcome, $\cont$. 
\mbinline{I would not say “naturally”: I was very surprised by this.
    I would have expected a command like return to just return \(\normal{\gvl}\)
    and to have a rule stating that if the current outcome~\(\outcome\) is not \(\cont\),
    then the call stack is inspected, and so on.
    It seems to me that you inlined the rule that I had in mind, which is fine.}
%The rules are given in Figure~\ref{fig:sem}. 




\begin{figure}
\begin{minipage}{0.45\textwidth}
\begin{minted}[fontsize=\scriptsize]{ocaml}
module type State = sig 
    (** Type of states *)
    type t
    (** Type of values *)
    type vt
    (** Type of actions *)
    type a

    val init     : t 
    val setVar   : t -> Var -> vt -> t 
    val setStore : t -> (Var, vt) Map -> t 
    val store    : t -> (Var, vt) Map 
    val ee       : t -> Expr.t -> vt 
    val ea       : a -> t -> vt -> (t * vt) list 
    val assume   : t -> vt -> (t * vt) list   
    val fresh    : t -> vt -> (t * vt) list 
    val symb     : t -> vt -> (t * vt) list 
end
\end{minted}
\end{minipage}
\begin{minipage}{0.45\textwidth}
\begin{minted}[fontsize=\scriptsize]{ocaml}
module type Allocator = sig 
    (** Type of allocation records *)
    type t 
    (** Type of values for allocation *)
    type vt 

    val alloc : t -> int -> (t * vt)
end
\end{minted}
\end{minipage}
\caption{OCaml State Signature}\label{fig:ocaml:state:sig}
\vspace{-10pt}
\end{figure}

\myparagraph{Implementation}
The \gil semantics is implemented as an OCaml functor parameterised by an 
OCaml module with type \texttt{State}, as given in Figure~\ref{fig:ocaml:state:sig} (left). 
The \texttt{State} module type precisely follows our formal definition of state 
module as in Definition~\ref{def:state:module}. 
Furthermore, the code of the \gil interpreter does also follow the formal definition 
of the semantics given in Figure~\ref{fig:sem}. 


\subsubsection{\gil Allocation}

In order to account for the generation of fresh values, be they locations or general values, we 
rely on the notion of allocator~\polish{\cite{??}}.
%
The generation of fresh values is a common source of technical clutter and is often 
omitted or hand-waved in the formal presentation of program analyses.
%
By providing a generator of fresh locations, \gillian relieves the user of the framework 
from having to reason explicitly about the generation of such values. 
\mbinline{This is the first occurence of \gillian in the text, but I assume that it will be referenced in the introduction.}

Informally, an allocator module $\allocator \in \allocators$ describes a set of allocators 
$\sset{\allocator}_\gval \ni \arec$, each generating fresh values taken from a given set $\gval$. 
Allocators can be ordered according to a pre-order $\allocle$ specified as part of the allocator module.  
Intuitively, $\arec_1 \allocle \arec_2$ holds if $\arec_1$ has allocated all the values allocated by 
$\arec_2$ and possibly more.  
Additionally, an allocator module is required to expose a function 
$\allocf : \sset{\allocator} \tmap \ints \tmap \power{\gval} \pmap \sset{\allocator} \times \gval$, 
written $\allocf(\arec, i, X)$, for generating a fresh value taken from 
$X \subseteq \gval$ and associate that value with the \emph{allocation site} uniquely identified by 
the integer $i$. 
The function $\allocf$ returns a pair consisting of the new allocator together with the 
created value. 

\begin{definition}[Allocator Module]
An allocator module $\allocator \in \allocators$ is a triple $\tup{\sset{\allocator}, \gval, \allocle}$ consisting of: 
\etag{1} a set $\sset{\allocator} \ni \arec$ of allocators,  
\etag{2} a set $\gval$ of values to allocate, and 
\etag{3} a pre-order $\allocle$ on  $\sset{\allocator}$. 
An allocator module additionally defines the following function for allocating fresh values:\\
\indent $\allocf : \sset{\allocator} \tmap \ints \tmap \power{\gval} \pmap \sset{\allocator} \times \gval$ 
\hfill  
($(\arec', \gvl) = \allocf(\arec, i, Y) \equiv \alloc{\arec}{i}{\arec', \gvl}{Y}$) \\
which satisfies the following constraints: \\ 
\begin{mathpar}
\inferrule[Monotonicity]{}{\alloc{\arec}{i}{\arec', \gvl}{Y} \implies \arec' \allocle \arec}
\and
\inferrule[Well-formedness]{}{\alloc{\arec}{i}{\arec', \gvl}{Y} \implies \gvl \in Y}
\end{mathpar}
\end{definition}

\subsection{\while: Syntax and Translation}\label{subsec:while:compiler}

Throughout the paper, we will illustrate how to use \gillian to obtain a compositional symbolic analysis for a simple \while language
with static objects reminiscent of that of~\cite{}. 
We start by showing how to compile \while to \gil by picking the appropriate actions 
for acting on \while states and making proper use of the \gil built-in facilities. 

The syntax of \while is given in the table below; it includes: the standard \while constructs 
(variable assignments, skip, sequence, if, and while); function calls and 
return statements; assume and assert statements for driving the symbolic analysis; 
and statements for operating on static objects (object creation, 
property look-up, property mutation, and object disposal). 

\begin{display}{\while: Syntax}
\begin{tabular}{l}
   %
   $\cw \in \cws \, \defeq \,  \x := \e \mid \wskip \mid \cw_1; \cw_2 \mid \wif{\e}{\cw_1}{\cw_2} \mid \wwhile{\e}{\cw} $  \\ 
   $\phantom{\cw \in \cws  \defeq \}} \mid \wreturn{\e} \mid \x := \fid(\e) \mid \wassume{\e} \mid \wassert{\e}$ \\ 
   $\phantom{\cw \in \cws  \defeq \}} \mid \x := \wobj{\prop_i: \e_i\mid_{i=1}^n} \mid \wlookup{\x}{\e}{\prop} \mid \wmutate{\e}{\prop}{\e'} \mid \wdispose{\e}$ 
 \end{tabular}
\end{display}

\begin{figure}
{\footnotesize
\begin{mathpar}
\inferrule[\textsc{Assignment}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\x := \e, \wpc) \semeq \\
      {\begin{array}{l}
        \wpc:  \x := \e  \\ 
         \nextpc{\wpc + 1}
       \end{array}} 
      \end{array}}
  }
%  
 \and 
 %
 \inferrule[\textsc{Skip}]
  {\wpc' = \wpc + 1}{
     {\begin{array}[t]{l}
      \compWhile(\wskip, \wpc) \semeq \\
      {\begin{array}{l}
        \wpc: \ifgoto{\true}{\wpc'} \\ 
         \nextpc{\wpc + 1}
       \end{array}} 
      \end{array}}
  }
 %
 \and 
 %
  \inferrule[\textsc{Return}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wreturn{\e}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \return{\e} \\  
         \nextpc{\wpc+1}
       \end{array}} 
      \end{array}}
  }
  %
 \and 
 %
   \inferrule[\textsc{Call}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\x := \fid(\e), \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \x := \fid{\e} \\  
         \nextpc{\wpc+1}
       \end{array}} 
      \end{array}}
  }
 %
 \and
 %
 \inferrule[\textsc{Sequence}]
  {
     \compWhile(\cw_1, \wpc) = (\lst{\cm}_1, \wpc_1) \\\\
     \compWhile(\cw_2, \wpc_1) = (\lst{\cm}_2, \wpc_2)
  }{
     {\begin{array}[t]{l}
      \compWhile(\cw_1; \cw_2, \wpc) \semeq \\
      {\begin{array}{l}
         \lst{\cm}_1 \\ 
         \lst{\cm}_2 \\ 
         \nextpc{\wpc_2 + 1}
       \end{array}} 
      \end{array}}
  }
%
\and 
%
  \inferrule[\textsc{If}]
  {
     \compWhile(\cw_1, \wpc+1) = (\lst{\cm}_1, \wpc_1) \\\\
     \compWhile(\cw_2, \wpc_1+1) = (\lst{\cm}_2, \wpc_2)
  }{
     {\begin{array}[t]{l}
      \compWhile(\wif{\e}{\cw_1}{\cw_2}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \ifgoto{(\gnot \, \e)}{(\wpc_1+1)} \\ 
         \lst{\cm}_1 \\ 
         \wpc_1: \ifgoto{\true}{\wpc_2} \\ 
         \lst{\cm}_2 \\ 
         \nextpc{\wpc_2}
       \end{array}} 
      \end{array}}
  }
  %
 \and 
 %
  \inferrule[\textsc{While}]
  {
     \compWhile(\cw, \wpc+1) = (\lst{\cm}, \wpc') 
  }{
     {\begin{array}[t]{l}
      \compWhile(\wwhile{\e}{\cw}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \ifgoto{(\gnot \, \e)}{(\wpc' +1)} \\ 
         \lst{\cm} \\ 
         \wpc': \ifgoto{\true}{\wpc} \\ 
         \nextpc{\wpc'+1}
       \end{array}} 
      \end{array}}
  }
%
\and 
%
\inferrule[\textsc{Assume}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wassume{\e}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \ifgoto{\e}{(\wpc + 2)} \\ 
          \wpc+1: \vanish \\
         \nextpc{\wpc + 2}
       \end{array}} 
      \end{array}}
  }
%
\and 
%
\inferrule[\textsc{Assert}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wassert{\e}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \ifgoto{\e}{(\wpc + 2)} \\ 
          \wpc+1: \fail{\true} \\
         \nextpc{\wpc + 2}
       \end{array}} 
      \end{array}}
  }
%
\and 
%
\inferrule[\textsc{New}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\x := \wobj{\prop_i: \e_i\mid_{i=1}^n}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \x :=  \fresh{} \\ 
          \wpc+i: \_ := \mutateAction(\litlst{\x, \prop_i, \e_i}) \mid_{i=1}^n \\
         \nextpc{\wpc + n + 1}
       \end{array}} 
      \end{array}}
  }
 %
 \and 
 %
 \inferrule[\textsc{Lookup}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wlookup{\x}{\e}{\prop}, \wpc) \semeq \\
      {\begin{array}{l}
          \wpc: \x := \lookupAction(\x, \prop) \\
         \nextpc{\wpc + 1}
       \end{array}} 
      \end{array}}
  }
  %
  \and 
  %
  \inferrule[\textsc{Mutate}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wmutate{\e_1}{\prop}{\e_2}, \wpc) \semeq \\
      {\begin{array}{l}
          \wpc: \_ := \mutateAction(\litlst{\e_1, \prop, \e_2}) \\
         \nextpc{\wpc + 1}
       \end{array}} 
      \end{array}}
  }
  %
  \and 
  %
    \inferrule[\textsc{Dispose}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wdispose{\e}, \wpc) \semeq \\
      {\begin{array}{l}
          \wpc: \_ := \disposeAction(\e) \\
         \nextpc{\wpc + 1}
       \end{array}} 
      \end{array}}
  }
 \end{mathpar}}
\caption{\while Compilation. $\compWhile : \cws \tmap \ints \tmap \litlst{\cmds{\actionswhile}} \times \ints$}
\label{while:compiler}
\end{figure}

\medskip
In order to compile \while to \gil, we first pick a set of actions $\actionswhile$ for acting on \while states, 
$\actionswhile = \lbrace \lookupAction, \mutateAction, \disposeAction \rbrace$. 
We do not pick an action for object creation, as we can make use of \gillian's built-in allocator for 
generating a fresh location and then use the action $\mutateAction$ to set the initial values of 
the properties of the new object. 

The \while-to-\gil compiler is given in Figure~\ref{while:compiler}. It is modelled as a function 
$\compWhile : \cws \tmap \ints \tmap \litlst{\cmds{\actionswhile}} \times \ints$, mapping a 
\while statement $\cw \in \cws$ and a positive integer $\wpc$, read \emph{program counter}, 
to a sequence of \gil commands and the next available program counter. 
For instance, if $\compWhile(\cw, \wpc) = (\lst{\cm}, \wpc')$, it follows that the while 
statement $\cw$ is compiled to the sequence of \gil commands given by $\lst{\cm}$ and 
that the commands in $\lst{\cm}$ are to be labelled with indexes $\wpc$ to $\wpc'-1$, 
meaning that $\wpc'$ is the next available index. 

The compilation rules are standard. 
For illustration purposes, we will explain the rules \textsc{Assume} and \textsc{Assert}.
The assume statement ($\wassume{\e}$) is compiled to a goto statement, 
($\ifgoto{\e}{(\wpc + 2)}$) that checks whether or not the assumed expression ($e$) 
is true; if it is, the control is transferred to the next available program counter ($\wpc + 2$) and 
the execution continues; if it is not, we make use of the \gil command $\vanish$ to 
silently terminate that execution. 
Similarly, the assert statement ($\wassert{\e}$) is compiled to a goto statement 
($\ifgoto{\e}{(\wpc + 2)}$) that checks whether or not the asserted expression ($\e$) 
is true; however, if $\e$ does not hold, we make use of the \gil command $\fail$ to cause 
the execution to terminate with an error. 



\subsection{Concrete versus Symbolic}

\begin{figure}
\begin{minipage}{0.45\textwidth}
\begin{minted}[fontsize=\scriptsize]{ocaml}
module type CMemory = sig 
    (** Type of concrete memories *)
    type t 
    (** Type of actions *)
    type a 
    (** Type of concrete values *)
    type vt = Val.t
    val ea : a -> t -> vt -> (t * vt) option 
end
\end{minted}
\medskip
\begin{minted}[fontsize=\scriptsize]{ocaml}
module CST 
  (CMem  : CMemory) 
  (Alloc : Allocator with type vt1 = Loc.t 
                      and type vt2 = Val.t) : 
    (State with type a = CMem.a) = struct 
    type vt = CMem.vt
    type mt = CMem.t 
    type t  = mt * vt Store * Alloc.t 
      ...
end 
\end{minted}
\end{minipage}
%
\begin{minipage}{0.45\textwidth}
\begin{minted}[fontsize=\scriptsize]{ocaml}
module type SMemory = sig 
    (** Type of concrete memories *)
    type t 
    (** Type of actions *)
    type a 
    (** Type of symbolic values *)
    type vt = LExpr.t
    val ea : a -> t -> vt -> vt -> (t * vt * vt) list  
end
\end{minted}
\medskip
\begin{minted}[fontsize=\scriptsize]{ocaml}
module SST 
  (SMem  : SMemory) 
  (Alloc : Allocator with type vt1 = Loc.t
                      and type vt2 = LVar.t) :
    (State with type a = SMem.a) = struct 
  type vt = LExpr.t
  type mt = SMem.t
  type at = Alloc.t 
  type t  = mt * vt Store * at * LExpr.t   
    ...
end 
\end{minted}
\end{minipage}
\caption{OCaml Concrete/Symbolic Memory Signatures}\label{fig:make:state}
\end{figure}

The variable store is kept as part of every \gil state. Hence, regardless of the target language, 
one can always think of a \gil state as being composed of a variable store together with a 
target language memory. 
Here, we show how to automatically lift a given memory to a \gil state by extending that
memory with both a variable store component and an allocator component.  
In particular, we show how this lifting can be achieved for concrete and symbolic memories, 
as formally described in Definition~\ref{def:memories}. 

While concrete memories store concrete values $\vl \in \vals$, symbolic memories store 
logical expressions $\sexp \in \sexps$, generated by the following grammar: 
$\sexp \in \sexps \ \defeq \ \vl \mid \lx \in \lxs \mid \unop{\sexp} \mid \binop{\sexp_1}{\sexp_2}$, 
where $\lx$ ranges over a set  $\lxs$ of \emph{logical variables}. 
In the following, we use $\pc \in \pcs \subset \sexps$ to range over the set of logical expressions that can be 
statically determined to have type Boolean. 

%Symbolic memories differ from a concrete memories in that they store symbolic values 
%instead of concrete values $\vl \in \vals$. Symbolic values are represented in \gillian 
%as logical expression $\sexp \in \sexps$, generated by the following grammar: 
%$\sexp \in \sexps \ \defeq \ \vl \mid \lx \in \xs \mid \unop{\sexp} \mid \binop{\sexp_1}{\sexp_2}$. 


%\begin{definition}[Logical Expressions/Logical Environment/Interpretation]
%Logical expressions $\sexp \in \sexps$ are given by the following grammar: 
%$$
%\sexp \in \sexps \ \defeq \ \vl \mid \lx \in \xs \mid \unop{\sexp} \mid \binop{\sexp_1}{\sexp_2}
%$$
%A logical environment $\lenv : \lxs \pmap \vals$ is a partial mapping from logical variables 
%to \gil values. The interpretation of a logical expression $\sexp$ with respect to a logical 
%environment $\lenv$, written $\seval{\sexp}{\lenv}$ is inductively defined as follows: 
%\begin{mathpar}
%  \inferrule[\textsc{Value}]
%  {}{\seval{\vl}{\lenv} \semeq \vl}
%  \and
%    \inferrule[\textsc{LVar}]
%      {}{\seval{\lx}{\lenv} \semeq \lenv(\lx)}
%   \and 
%    \inferrule[\textsc{UnOp}]
%      {\seval{\sexp}{\lenv} = \vl}
%      {\seval{\unop{\sexp}}{\lenv} \semeq \sunop{\vl}}
%   \and
%    \inferrule[\textsc{BinOp}]
%      {
%        \seval{\sexp_1}{\lenv} = \vl_1
%        \and
%        \seval{\sexp_2}{\lenv} = \vl_2
%       }{\seval{\binop{\sexp_1}{\sexp_2}}{\lenv} \semeq \sbinop{\vl_1}{\vl_2}}
%\end{mathpar}
%\end{definition}


\begin{definition}[Concrete/Symbolic Memory Module]\label{def:memories}
A concrete/symbolic memory module $\cmemory \in \cmemories$/$\smemory \in \smemories$ 
is a pair $\tup{\sset{\cmemory}, \actions}$/$\tup{\sset{\smemory}, \actions}$,
consisting of a set of concrete/symbolic memories $\sset{\cmemory}$/$\sset{\smemory}$ and a set of actions $\actions$. 
A concrete/symbolic memory module additionally defines a function $\cea$/$\sea$ for acting 
on memories with the following type signatures: \\
\indent $\cea : \actions \tmap \sset{\cmemory} \tmap \vals \pmap \sset{\cmemory} \times \vals$  
\hfill (\emph{notation:} ${\kwT{ea}}(\act, \cmem, \vl) \equiv \cmem.\act(\vl)$)
\\ 
\indent $\sea : \actions \tmap \sset{\smemory} \tmap \sexps \tmap \pcs \pmap \power{\sset{\smemory} \times \sexps \times \pcs}$ \\ 
$\phantom{x}$ \hfill 
  (\emph{notation:} $(\smem', \sexp', \pc') \in \hat{\kwT{ea}}(\act, \smem, \sexp, \pc) \equiv \action{\smem}{\act}{\sexp, \pc}{(\smem', \sexp', \pc')}$)
\end{definition}

%\begin{definition}[Symbolic Memory Module]
%A symbolic memory module $\smemory \in \smemories$ is a triple $\tup{\sset{\smemory}, \actions, \sea}$
%consisting of: \etag{1} a set of symbolic memories $\sset{\smemory}$, \etag{2} a set of actions $\actions$, 
%and \etag{3} a function:
%
%$\sea : \actions \tmap \sset{\smemory} \tmap \sexps \tmap \pcs \pmap \power{\sset{\smemory} \times \sexps \times \pcs}$ \\
% $\phantom{xxx} \quad$ 
% 
%for acting on memories. 
%\end{definition}

%\begin{definition}[Concrete/Symbolic Memory Module]\label{def:memories}
%A concrete memory module $\cmemory \in \cmemories$ is a triple $\tup{\sset{\cmemory}, \actions, \cea}$
%consisting of: \etag{1} a set of concrete memories $\sset{\cmemory}$, \etag{2} a set of actions $\actions$, 
%and \etag{3} a function $\cea : \actions \tmap \sset{\cmemory} \tmap \vals \pmap \sset{\cmemory} \times \vals$ 
%for acting on memories. 
%\end{definition}
%
%\begin{definition}[Symbolic Memory Module]
%A symbolic memory module $\smemory \in \smemories$ is a triple $\tup{\sset{\smemory}, \actions, \sea}$
%consisting of: \etag{1} a set of symbolic memories $\sset{\smemory}$, \etag{2} a set of actions $\actions$, 
%and \etag{3} a function:
%
%$\sea : \actions \tmap \sset{\smemory} \tmap \sexps \tmap \pcs \pmap \power{\sset{\smemory} \times \sexps \times \pcs}$ \\
% $\phantom{xxx} \quad$ (\emph{notation:} $(\smem', \sexp', \pc') \in \hat{\kwT{ea}}(\act, \smem, \sexp, \pc) \equiv \action{\smem}{\act}{\sexp, \pc}{(\smem', \sexp', \pc')}$)
% 
%for acting on memories. 
%\end{definition}

Given a concrete memory, $\cmem \in \sset{\cmemory}$, we construct a concrete state $\st$ by \polish{pairing up} 
$\cmem$ with a concrete store $\sto : \xs \pmap \vals$ and a concrete allocator $\arec \in \sset{\allocator}_{\vals}$. 
Analogously, given a symbolic memory, $\smem \in \sset{\smemory}$, we construct a symbolic state $\sst$ by 
\polish{pairing up} $\smem$ with a symbolic store $\ssto : \xs \pmap \sexps$ and a symbolic allocator 
$\sarec \in \sset{\allocator}_{\sexps}$. However, in the symbolic case, we also include in the constructed 
state, $\sst$, a logical expression $\pc \in \pcs$, referred to as the \emph{path condition} of $\sst$. 
Path conditions~\cite{} bookeep the constraints on the symbolic variables that led the execution to the 
current symbolic state. 
%
The liftings from concrete and symbolic memories to concrete and symbolic states are formally described in 
Definitions~\ref{def:concrete:lifting} and~\ref{def:symbolic:lifting}, respectively.

\begin{definition}[Concrete State Transformer (CST)]\label{def:concrete:lifting}
Given an allocator $\allocator = \tup{\sset{\allocator}, \vals, \allocle}$, the 
concrete state constructor $\cstateConstr : \cmemories \tmap \gstates$ is defined as  
$\cstateConstr(\tup{\sset{\cmemory}, \actions}) \semeq \tup{\sset{\gstate}, \vals, \actions  \dunion \actionsZ}$,
where: 

{\small
\begin{tabular}{lll}
   \multicolumn{3}{l}{\mybullet $\sset{\gstate} = \sset{\cmemory} \times \pfunset{\xs}{\vals} \times \sset{\allocator}_{\vals}$} \\ 
  %
  \mybullet $\kwT{setVar}(\tup{\cmem, \sto, \arec}, \x, \vl)$ 
       & $\semeq$ & 
       $\tup{\cmem, \sto[\x \mapsto \vl], \arec}$ \\ 
  %
  \mybullet $\kwT{setStore}(\tup{\cmem, \_, \arec}, \sto)$
     & $\semeq$ & 
     $\tup{\cmem, \sto, \arec}$ \\ 
  %
  \mybullet $\kwT{store}(\tup{\_, \sto, \_})$
    & $\semeq$ & 
    $\sto$ \\
  %
  \mybullet $\kwT{ee}(\tup{\_, \sto, \_}, \e)$
    & $\semeq$ & 
    $\ceval{\e}{\sto}$ \\
 %
 \mybullet $\kwT{ea}(\act, \tup{\cmem, \sto, \arec}, \vl)$
    & $\semeq$ & 
    $\lbrace (\tup{\cmem', \sto, \arec}, \vl') \mid (\cmem', \vl') = \cea(\act, \cmem, \vl) \rbrace$ \\
  %
   \mybullet $\kwT{assume}(\st, \vl)$
    & $\semeq$ & 
    $\lbrace (\st, \vl) \mid \vl = \true \rbrace$ \\
   %
    \mybullet $\kwT{fresh}(\tup{\cmem, \sto, \arec}, i)$
    & $\semeq$ &
     $\lbrace (\tup{\cmem, \sto, \arec'}, \loc) \mid \alloc{\arec}{i}{\arec', \loc}{\locs} \rbrace $ \\
    %
    \mybullet $\kwT{symb}(\tup{\cmem, \sto, \arec}, i)$
    & $\semeq$ &
     $\lbrace (\tup{\smem, \ssto, \arec'}, \vl) \mid \alloc{\arec}{i}{\arec', \vl}{\vals} \rbrace $ \\
    
%   \mybullet $\kwT{fresh/symb}(\tup{\cmem, \sto, \freeRec, \freeCnt}, i)$
%    & $\semeq$ & 
%    $\lbrace (\tup{\cmem, \sto, \freeRec, \freeCnt[i \mapsto \freeCnt(i){+}1]}, \vl) \mid \vl = \freeRec(i, \freeCnt(i)) \rbrace $ \\
%  %
%   \mybullet $\kwT{fresh}(\tup{\cmem, \sto, \freeRec, \freeCnt}, i)$
%    & $\semeq$ & 
%    $\left\{ {\begin{array}{l}
%          (\tup{\cmem, \sto, \freeRec[(i, j) \mapsto \loc], \freeCnt[i \mapsto j{+}1]}, \loc) \\ 
%           \quad \mid j = \freeCnt(i) \gand (i, j) \not\in \domain(\freeRec) \gand \loc \not\in \rng(\freeRec) 
%           \end{array}} \right\}$ \\
%  %
%   \mybullet $\kwT{symb}(\tup{\cmem, \sto, \freeRec, \freeCnt}, i)$
%    & $\semeq$ & 
%    $\left\{ {\begin{array}{l}
%          (\tup{\cmem, \sto, \freeRec[(i, j) \mapsto \vl], \freeCnt[i \mapsto j{+}1]}, \vl) \\ 
%           \quad \mid j = \freeCnt(i) \gand (i, j) \not\in \domain(\freeRec) \gand \vl \not\in \rng(\freeRec) 
%           \end{array}} \right\}$ \\
\end{tabular}}
\end{definition}


\begin{definition}[Symbolic State Transformer (SST)]\label{def:symbolic:lifting}
Given an allocator $\hat\allocator = \tup{\sset{\hat\allocator}, \sexps, \allocle}$, the 
symbolic state constructor $\sstateConstr : \smemories \tmap \gstates$ is defined as 
$\sstateConstr(\tup{\sset{\smemory}, \actions}) \semeq \tup{\gsstate, \sexps, \actions  \dunion \actionsZ}$,
where: 

{\small
\begin{tabular}{lll}
   \multicolumn{3}{l}{\mybullet $\gsstate = \sset{\smemory} \times \pfunset{\xs}{\sexps} \times \sset{\allocator}_{\sexps} \times \pcs$} \\ 
  %
  \mybullet $\kwT{setVar}(\tup{\smem, \ssto, \sarec, \pc}, \x, \sexp)$ 
       & $\semeq$ & 
       $\tup{\smem, \ssto[\x \mapsto \sexp], \sarec, \pc}$ \\ 
  %
  \mybullet $\kwT{setStore}(\tup{\smem, \_, \sarec, \pc}, \ssto)$
     & $\semeq$ & 
     $\tup{\smem, \ssto, \sarec, \pc}$ \\ 
  %
  \mybullet $\kwT{store}(\tup{\_, \ssto, \_, \_})$
    & $\semeq$ & 
    $\ssto$ \\
  %
  \mybullet $\kwT{ee}(\tup{\_, \ssto, \_, \_}, \e)$
    & $\semeq$ & 
    $\ssto(\e)$ \\
 %
 \mybullet $\kwT{ea}(\act, \tup{\smem, \ssto, \sarec, \pc}, \sexp)$
    & $\semeq$ & 
    $\lbrace (\tup{\smem', \ssto, \sarec, \pc \, \wedge \pc'}, \sexp') \mid (\smem', \sexp', \pc') \in \sea(\act, \smem, \sexp) \rbrace$ \\
  %
   \mybullet $\kwT{assume}(\tup{\smem, \ssto, \sarec, \pc}, \pc')$
    & $\semeq$ & 
    $\lbrace (\tup{\smem, \ssto, \sarec, \pc \gand \pc'}, \true) \mid \pc \gand \pc' \, \text{not \unsat} \rbrace$ \\%, if $\pc \gand \pc'$ \sat \\
  %
  \mybullet $\kwT{fresh}(\tup{\smem, \ssto, \sarec, \pc}, i)$
    & $\semeq$ &
    $\lbrace (\tup{\cmem, \sto, \sarec', \pc}, \loc) \mid \alloc{\sarec}{i}{\sarec', \loc}{\locs} \rbrace $ \\
      %
  \mybullet $\kwT{symb}(\tup{\smem, \ssto, \sarec, \pc}, i)$
    & $\semeq$ &
    $\lbrace (\tup{\cmem, \sto, \sarec', \pc}, \loc) \mid \alloc{\sarec}{i}{\sarec', \loc}{\lxs} \rbrace $ \\
  
 %  \mybullet $\kwT{assume}(\tup{\_, \_, \pc, \_, \_}, \pc')$
  %  & $\semeq$ & 
  %  $\lbrace \rbrace$, if $\pc \gand \pc'$ \\
  %
%   \mybullet $\kwT{fresh/symb}(\tup{\smem, \ssto, \pc, \sfreeRec, \sfreeCnt}, i)$
%    & $\semeq$ & 
%    $\lbrace (\tup{\smem, \ssto, \pc, \sfreeRec, \sfreeCnt[i \mapsto \sfreeCnt(i){+}1]}, \sexp) \mid \sexp = \sfreeRec(i, \sfreeCnt(i)) \rbrace$ \\ 
%  %
%   \mybullet $\kwT{fresh}(\tup{\smem, \ssto, \pc, \sfreeRec, \sfreeCnt}, \loc)$
%    & $\semeq$ & 
%      $\left\{ {\begin{array}{l}
%          (\tup{\smem, \ssto, \pc, \sfreeRec[(i, j) \mapsto \loc], \sfreeCnt[i \mapsto j{+}1]}, \loc) \\ 
%           \quad \mid j = \sfreeCnt(i) \gand (i, j) \not\in \domain(\sfreeRec) \gand \loc \not\in \rng(\sfreeRec) 
%           \end{array}} \right\}$ \\
%  %
%   \mybullet $\kwT{symb}(\tup{\smem, \ssto, \pc, \sfreeRec, \sfreeCnt}, \lx)$
%    & $\semeq$ & 
%     $\left\{ {\begin{array}{l}
%          (\tup{\smem, \ssto, \sfreeRec[(i, j) \mapsto \lx], \freeCnt[i \mapsto j{+}1]}, \lx) \\ 
%           \quad \mid j = \sfreeCnt(i) \gand (i, j) \not\in \domain(\sfreeRec) \gand \lx \not\in \rng(\sfreeRec) 
%           \end{array}} \right\}$ \\
\end{tabular}}
\end{definition}

The concrete/symbolic lifting constructs the functions that a state module exposes using the function 
$\kwT{ea}$ (\emph{execute action}) of the parameter concrete/symbolic memory and the function 
$\kwT{alloc}$ of the parameter concrete/symbolic allocator. 
In both cases, the construction of $\kwT{setVar}$, $\kwT{setStore}$, and 
 $\kwT{store}$ is straightforward. The remaining cases are described below. \\
% 
\indent \prooflab{EvalExpr} The function $\kwT{ee}$ evaluates the given expression in the store of the 
state. In the concrete case, expression evaluation is performed concretely (we use $\ceval{\e}{\sto}$ to denote the
standard expression evaluation of $\e$ with respect to $\sto$). In the symbolic case, expression
evaluation amounts to substituting all the program variables in $\e$ with their associated logical 
expressions given by the store (we use $\ssto(\e)$ to denote that substitution).  \\
%
\indent \prooflab{Action} The function $\kwT{ea}$ applies the given action to the memory 
of the state. This amounts to calling the function $\kwT{ea}$ of the parameter memory.
% and wrapping the result with the current store and allocator (and path condition, in the symbolic case). 
Observe that symbolic actions, unlike concrete actions, may branch. For this reason, they additionally 
generate a logical expression, $\pc'$, describing the conditions under which the chosen 
branch is taken. Hence, to obtain the new path condition, we conjunct $\pc'$ with the path 
condition $\pc$ of the original state. \\ 
%
\indent \prooflab{Assume} The function $\kwT{assume}$ generates a set of states in which 
the given value \emph{holds}. 
In the concrete case, we return the singleton set containing the original state when given the value $\true$
 and the empty set otherwise. 
In the symbolic case, we simply conjunct the given logical expression with the current path condition.
Note that if we can prove that the new path condition is $\unsat$, we also generate the empty set. \\
%
\indent \prooflab{Fresh/Symb} The function $\kwT{fresh}$/$\kwT{symb}$ generates a fresh location/value 
using the parameter allocator. We use the arrow parameter of the allocator to indicate the set from which to pick 
the freshly generated value: $\kwT{fresh}$ picks a location and $\kwT{symb}$ picks an \polish{arbitrary} value. 
While concrete values coincide with \gil values in $\vl \in \vals$, symbolic values are logical expressions 
$\sexp \in \sexps$. 
\polish{Hence, when generating a fresh symbolic value, we simply pick a fresh logical variable.}

%In the concrete state, this evaluation is done concretely (we use $\ceval{\e}{\sto}$ to denote the
%standard expression evaluation of $\e$ with respect to $\sto$). In the symbolic case, expression
%evaluation amounts to substituting all the program variables in $\e$ with their associated logical 
%expressions given by the symbolic store (we use $\ssto(\e)$ to denote that substitution).  



\begin{figure}[t!]

\begin{minipage}{0.35\textwidth}
{\small
\begin{mathpar}
%\inferrule[Concrete Memory Type]
%{}{\cmem \in \wcmems: \locs \tmap \strs \pmap \vals}
%\\
%\inferrule[Concrete Action Type]
%{}{\cea : \actionswhile \tmap \wcmems \tmap \vals \pmap \wcmems \times \vals }
%\\
\inferrule[C-Lookup]
  {\cmem = \_ \dunion \wcell{\loc}{\prop}{\vl}}
  {\action{\cmem}{\lookupAction}{\litlst{\loc, \prop}}{(\cmem, \vl)}} 
 \\
\inferrule[C-Mutate]
  {
    \cmem = \cmem' \dunion \wcell{\loc}{\prop}{\_}
    \\\\
    \cmem'' = \cmem' \dunion \wcell{\loc}{\prop}{\vl}
  }{\action{\cmem}{\mutateAction}{\litlst{\loc, \prop, \vl}}{(\cmem'', \vl)}} 
 \\
\inferrule[C-Dispose]
  {
    \memproj{\cmem}{\loc} = (\_, \cmem')
  }{\action{\cmem}{\disposeAction}{\loc}{(\cmem', \true)}} 
%\\ 
%\inferrule[C-Proj Empty]{}
%  {\memproj{\emptymem}{\loc} \ \semeq \, (\emptymem, \emptymem)}  
%\\
%\inferrule[C-Proj Cell - 1]
%  { \loc' = \loc }
%  {\memproj{(\wcell{\loc'}{\prop}{\vl})}{\loc} \ \semeq \, (\wcell{\loc}{\prop}{\vl}, \emptymem)}  
%\\ 
%\inferrule[C-Proj Cell - 2]
%  {\loc' \neq \loc}
%  {\memproj{(\wcell{\loc'}{\prop}{\vl})}{\loc} \ \semeq \, (\emptymem, \wcell{\loc'}{\prop}{\vl})}  
%\\ 
%\inferrule[C-Proj Union]
%  {
%    \memproj{\cmem_1}{\loc} = (\cmem_1', \cmem_1'') \and
%    \memproj{\cmem_2}{\loc} = (\cmem_2', \cmem_2'')
%  }{\memproj{\cmem_1 \dunion \cmem_2}{\loc} \ \semeq \, (\cmem_1' \dunion \cmem_2', \cmem_1'' \dunion \cmem_2'')}  
\end{mathpar}}
\end{minipage}
\begin{minipage}{0.55\textwidth}
{\small
\begin{mathpar}
%\inferrule[Symbolic Memory Type]
%{}{\smem \in \wsmems: \sexps \tmap \strs \pmap \sexps}
%\\
%\inferrule[Symbolic Action Type]
%{}{\sea : \actionswhile \tmap \wsmems \tmap \sexps \tmap \pcs \pmap \power{\wsmems \times \sexps}}
%\\
\inferrule[S-Lookup]
  {
     \smem = \_ \dunion \wcell{\sexp'}{\prop}{\sexp_v}
     \and 
     \pc \vdash \sexp = \sexp' 
  }{\action{\smem}{\lookupAction}{\litlst{\sexp, \prop}, \pc}{\litset{(\smem, \sexp_v, \true)}}} 
 \\
\inferrule[S-Mutate]
  {
    \smem = \smem' \dunion \wcell{\sexp''}{\prop}{\_}
    \and 
    \pc \vdash \sexp = \sexp'' 
    \\\\
    \smem'' = \smem' \dunion \wcell{\sexp''}{\prop}{\sexp'}
  }{\action{\smem}{\mutateAction}{\litlst{\sexp, \prop, \sexp'}, \pc}{\litset{(\smem'', \sexp'', \true)}}} 
 \\
\inferrule[S-Dispose]
  {
    \memproj{\smem}{\sexp, \pc} = (\_, \smem')
  }{\action{\smem}{\disposeAction}{\sexp, \pc}{\litset{(\smem', \true, \true)}}}
%\\ 
%\inferrule[S-Proj Empty]{}
%  {\memproj{\emptymem}{\sexp, \pc} \ \semeq \, (\emptymem, \emptymem)}  
%\\
%\inferrule[S-Proj Cell - 1]
%  { \pc \vdash \sexp = \sexp'}
%  {\memproj{(\wcell{\sexp'}{\prop}{\sexp''})}{\sexp} \ \semeq \, (\wcell{\sexp}{\prop}{\sexp''}, \emptymem)}  
%\\ 
%\inferrule[S-Proj Cell - 2]
%  { \pc \vdash \sexp \neq \sexp'}
%  {\memproj{(\wcell{\sexp'}{\prop}{\sexp''})}{\sexp} \ \semeq \, (\emptymem, \wcell{\sexp'}{\prop}{\sexp''})}  
%\\ 
%\inferrule[C-Proj Union]
%  {
%    \memproj{\smem_1}{\sexp, \pc} = (\smem_1', \smem_1'') \and
%    \memproj{\smem_2}{\sexp, \pc} = (\smem_2', \smem_2'')
%  }{\memproj{\smem_1 \dunion \smem_2}{\sexp, \pc} \ \semeq \, (\smem_1' \dunion \smem_2', \smem_1'' \dunion \smem_2'')}  
\end{mathpar}}
\end{minipage}
%\begin{mathpar}
% \inferrule[C-Projection]
% {}{
% {\begin{array}{l}
%   \memproj{\emptymem}{\loc} \ \semeq \, (\emptymem, \emptymem) \\
%   \memproj{(\wcell{\loc}{\prop}{\vl})}{\loc} \ \semeq \, (\wcell{\loc}{\prop}{\vl}, \emptymem) \\
%   \memproj{(\wcell{\loc'}{\prop}{\vl})}{\loc} \ \semeq \, (\emptymem, \wcell{\loc}{\prop}{\vl}) \text{ if } \loc' \neq \loc
% \end{array}}}
%\end{mathpar}
\vspace{-10pt}
\caption{\while: Concrete and Symbolic Memories}\label{fig:while:memories}\vspace{-10pt}
\end{figure}


\myparagraph{Implementation}
The concrete and symbolic state transformers are implemented as OCaml functors,
respectively parameterised by an OCaml module with type \texttt{CMemory} and an OCaml
module with type \texttt{SMemory}, as given in Figure~\ref{fig:make:state}. 
Both functors are additionally parameterised by a module with type \texttt{Allocator}
for the generation of fresh values. % corresponding to the allocator. 
The \texttt{CMemory} and \texttt{SMemory} module types precisely follow our formal characterization of 
concrete and symbolic state modules as per Definition~\ref{def:memories}. 
Furthermore, the functors \texttt{CST} and \texttt{SST} do also follow the concrete and symbolic 
liftings described in Definitions~\ref{def:concrete:lifting} and~\ref{def:symbolic:lifting}. 
For instance, one can easily check that their respective carrier types (both called \texttt{t}) 
precisely match the carrier sets of the \emph{lifted} states. 


\subsection{\while: Concrete and Symbolic Memories}

We show how to obtain a concrete/symbolic interpreter\footnote{\polish{Should I say semantics or interpreter?}}
for \while by combining the 
\while-to-\gil compiler given in \S\ref{subsec:while:compiler} with a concrete/symbolic \while memory module. 
In practice, in order to obtain an off-the-shelf fully functional interpreter (be it concrete or symbolic), 
the user of \gillian simply needs to provide a compiler from the target language to \gil together 
with an implementation of the appropriate memory module.  
For a concrete interpreter, they need to provide a concrete memory; \emph{mutatis mutandis} 
for a symbolic interpreter. 
Unsurprisingly, the actions of the memory module must match those of the syntax 
(used by the compiled code).

The first step towards defining a memory module is to pick the carrier set of the module, 
in this case: the set of \while memories. 
We define a concrete \while memory to be a partial mapping from locations and strings 
(corresponding to property names) to values; formally: $\cmem \in \wcmems: \locs \times \strs \pmap \vals$. 
Analogously, we define a symbolic memory to be a partial mapping from 
logical expressions and strings to logical expressions; formally: $\smem \in \wsmems: \sexps \times \strs \pmap \sexps$. 
Property names are not lifted to logical expressions in the symbolic case, since the \while statements
that act on objects properties do not allow the property name to be resolved dynamically. 

Having chosen the symbolic and concrete carrier sets, we can now define the functions $\cea$ and $\sea$ for acting 
on concrete and symbolic memories, respectively. 
In particular, these functions must support the actions 
$\actionswhile = \lbrace \lookupAction, \mutateAction, \disposeAction \rbrace$ 
introduced in \S\ref{subsec:while:compiler}.
The definition of the \while concrete/symbolic actions is given in Figure~\ref{fig:while:memories}
(concrete on the left and symbolic on the right). 
The definition is standard. 
Below, we describe the rules \prooflab{C-Dispose} and \prooflab{S-Dispose}.\\
% 
\indent \prooflab{C-Dispose} In order to dispose  of the object at location $\loc$, we make use 
of the projection operator $\memproj{(.)}{\loc}$ to split the given memory $\cmem$ into a pair  
$(\cmem'', \cmem')$, where $\cmem''$ contains the memory cells at location $\loc$ and 
$\cmem'$ contains the others. The action returns $\cmem'$ and the value $\true$. 
The value $\true$ is returned to comply with the expected type of 
$\cea$; it is not used by the compiled code. \\
%
\indent \prooflab{S-Dispose} This rule is analogous to \prooflab{C-Dispose}. 
It starts by splitting the symbolic memory $\smem$ into a pair 
$(\smem'', \smem')$, where $\smem''$ contains the memory cells at 
the location \emph{denoted by} $\sexp$ and $\smem'$ contains the others.
However, 
the symbolic projection operator  $\memproj{(.)}{\sexp, \pc}$ makes use of the 
current path condition $\pc$ to determine which symbolic cells denote the same 
location as $\sexp$. 
The action returns $\cmem'$, the value $\true$, and the path condition $\true$. 
The returned path condition is $\true$ to indicate that the action does not branch
and, therefore, the path condition of the corresponding state does not have 
to be~updated. 

\myparagraph{Implementation} \gillian comes with a first order solver 
for discharging entailment questions involving \gil logical expressions, such as 
$\pc \vdash \sexp = \sexp'$ in the Rule \prooflab{S-Lookup}. 
%
This makes it easy for the user of the framework to swiftly develop new memory modules, 
as he/she only needs to define the operations that interact with their memory
type, while relying on the framework for solving the first order queries that those operations beget.\footnote{\polish{I 
want to say something about Z3 and what do we actually support.}}
%The first order solver is simply a front-end to Z3~\cite{}. 

\subsection{Parametric Soundness}

Proving the soundness of a symbolic analysis is a time-consuming task 
often requiring a considerable number of auxiliary lemmas and definitions.
The complexity, and sheer size, of such proofs rapidly becomes unwieldy, 
as we consider real programming languages with multiple program constructs and 
complex runtime environments.  
This is, however, unfortunate, as it detracts from mathematical rigour in favour of 
less time consuming, but also less trustworthy, informal arguments. 
One of the main goals of \gillian is to streamline the development of soundness 
proofs for the instantiations of the framework, by focusing the \emph{proof effort}
of the user on the target language memory and the actions that it exposes. 

Our general proof infrastructure consists of 

\begin{definition}[Restriction Operator]
$\phantom{x}$
\begin{itemize}
  \item A \emph{restriction} operator $\frestriction : X \tmap X \pmap X$  on a set $X$, written $\rfun{x_1}{x_2}$ for 
   $\frestriction\!(x_1, x_2)$, is a binary \underline{associative} function satisfying the following properties: 
  {
   \begin{mathpar}
     \inferrule[Idempotence]{}{\rfun{x}{x} = x}
     \and
     \inferrule[Right Commutativity]{}{\rfun{x_1}{(\rfun{x_2}{x_3})} = \rfun{x_1}{(\rfun{x_3}{x_2})}}
     %\inferrule[Associativity]{}{\rfun{x_1}{(\rfun{x_2}{x_3})} = \rfun{(\rfun{x_1}{x_2})}{x_3}}
     \and
     \inferrule[Weakening]{}{x \rleq (\rfun{x_1}{x_2}) \implies x \rleq x_1 \, \wedge \, x \rleq x_2}
   \end{mathpar}}
   where: $x_1 \rleq x_2 \iff \rfun{x_1}{x_2} = x_1$. 
  \item A restriction operator on $X$,  $\frestriction : X \tmap X \pmap X$, is said to be \emph{consistent} with a given  
      pre-order $(X, \leq)$ if and only if the following constraints hold: 
    {\begin{mathpar}
        \inferrule[Consistency - 1]{}{\rfun{x_1}{x_2} \, \leq \, x_1}
        \qquad 
        \inferrule[Consistency - 2]{}{x_1 \leq x_2 \implies x_1 \rleq x_2}
        \qquad 
        \inferrule[Strengthening]{}{x_1 \leq x_1' \, \wedge \, x_2 \rleq x_2' \implies \rfun{x_1}{x_2} \, \leq \, \rfun{x_1'}{x_2'}}
        %
     \end{mathpar}}
\end{itemize}
\end{definition}


\begin{definition}[State/Configuration Restriction]
A restriction operator $\frestriction : \sset{\gstate} \tmap \sset{\gstate} \pmap \sset{\gstate}$ is said to be \emph{preserved} 
by a state module $\gstate = \tup{\sset{\gstate}, \gval, \actions}$ if and only if the following hold: 
\begin{mathpar}
     \inferrule[SetVar]{}{\st.\kwT{setVar}(\x, \vl) = \st' \implies \st' \rleq \st}
      \and
     \inferrule[SetStore]{}{\st.\kwT{setStore}(\sto) = \st' \implies \st' \rleq \st}
     \\
     \inferrule[Action]{}{\action{\st}{\act}{v}{(\st', -)} \implies \st' \rleq \st}
   \end{mathpar}
Restriction operators are extended from states to configurations in the standard way: 
$$
\rfun{\tup{\prog, \st_1, \cs_1, i}}{\tup{\prog, \st_2, \cs_2, j}} \semeq \tup{\prog, \rfun{\st_1}{\st_2}, \cs_1, i}
$$
\emph{Notation:} In the following, we say that $\frestriction$ is a restriction operator on 
$\gstate = \tup{\sset{\gstate}, \gval, \actions}$, if $\frestriction$ is a restriction 
operator on $\sset{\gstate}$ and $\frestriction$ is preserved by $\gstate$. 
\end{definition}

\begin{definition}[Induced Pre-Order] 
Given a relation $\rel \in X \times Y$ between two sets $X$ and $Y$, the pre-order 
on $X$ induced by $\rel$, $(X, \leq_{\rel})$, is defined as follows: 
$$x_1 \leq_{\rel} x_2 \iff \lbrace y \mid x_1 \, \rel \, y \rbrace \subseteq \lbrace y \mid x_2 \, \rel \, y \rbrace$$
\end{definition}

\begin{definition}[Soundness Criterion]
Given two state modules $\gstate_1 = \tup{\sset{\gstate_1}, \gval_1, \actions}$ and $\gstate_2 = \tup{\sset{\gstate_2}, \gval_2, \actions}$, 
a soundness criterion $\soundnessCriterion$ for $\gstate_1$ in terms of $\gstate_2$ is a triple
$\tup{\frestriction, \stRel, \vlRel}$, consisting of: 
\etag{1} a restriction operator $\frestriction$ on $\gstate_1$, 
\etag{2} a binary relation $\stRel \, \subseteq \sset{\gstate_1} \times \sset{\gstate_2}$ between $\sset{\gstate_1}$ and $\sset{\gstate_2}$, and 
\etag{3} a ternary relation $\vlRel \subseteq \sset{\gstate_1} \times \gval_1 \times \gval_2$ between  $\sset{\gstate_1}$, $\gval_1$, and $\gval_2$, 
such that $\frestriction$ is consistent with the pre-order induced by $\stRel$, $\leq$, and the following constraints hold: 
{\small
\begin{mathpar}
     %
     \inferrule[Store]{}{\vlR{\st_1}{\st_1.\kwT{store}}{\st_2.\kwT{store}}}
     %
     \qquad 
     %
     \inferrule[EvalExpr]{}{\leqStR{\st_1}{\st_1'}  \gand \stR{\st_1}{\st_2} 
            \implies \vlR{\rfun{\st_1' }{\st_1}}{\ee{\st_1'}{\e}}{\ee{\st_2}{\e}}}
     %
     \and
      \inferrule[SetVar]{}{
        {\begin{array}{l}
             \leqStR{\st_1}{\st_1'} \gand \stR{\st_1}{\st_2}  \gand \vlR{\st_1}{\vl_1}{\vl_2} \\
              \quad \implies \stR{\rfun{\st_1'.\kwT{setVar}(\x, \vl_1)}{\st_1}}{\st_2.\kwT{setVar}(\x, \vl_2)}
         \end{array}}}
     %
     \qquad 
     %
     \inferrule[SetStore]{}{
       {\begin{array}{l}
         \leqStR{\st_1}{\st_1'} \gand \stR{\st_1}{\st_2}  \gand \vlR{\st_1}{\sto_1}{\sto_2} \\
            \quad  \implies  \stR{\rfun{\st_1'.\kwT{setStore}(\sto_1)}{\st_1}}{\st_2.\kwT{setStore}(\sto_2)}
        \end{array}}}
     %
    \and 
    %
     \inferrule[Action]{}{\action{\st_1'}{\act}{\vl_1}{(\st_1'', \vl_1')} \gand \leqStR{\st_1}{\rfun{\st_1'}{\st_1''}} \gand \ \stR{\st_1}{\st_2} \gand  \vlR{\st_1}{\vl_1}{\vl_2} \\
            \qquad \implies \exists \, \st_2', \vl_2' \, . \, \action{\st_2}{\act}{\vl_2}{(\st_2', \vl_2')} \gand \stR{\rfun{\st_1'}{\st_1}}{\st_2'} \gand  \vlR{\rfun{\st_1'}{\st_1}}{\vl_1'}{\vl_2'}}
     %
     \and
     %
     \inferrule[Weakening]{}{
        \st_1 \rleq \st_1' \gand \vlR{\st_1}{\vl_1}{\vl_2} \implies \vlR{\st_1'}{\vl_1}{\vl_2}
     }
  \end{mathpar}}
 where $\vlR{\st}{\sto_1}{\sto_2}$ is shorthand for: $\domain(\sto_1) = \domain(\sto_2) = X$ and $\forall \x \in X \, . \, \vlR{\st}{\sto_1(\x)}{\sto_2(\x)}$.
\end{definition}


\begin{definition}[Soundness Criterion - CallStacks and Configurations]
Let $\soundnessCriterion = \tup{\frestriction, \stRel, \vlRel}$ be a soundness criterion
 for $\gstate_1 = \tup{\sset{\gstate_1}, \gval_1, \actions}$ in terms of $\gstate_2 = \tup{\sset{\gstate_2}, \gval_2, \actions}$
 and $\leq$ the pre-order induced by $\stRel$.
 \begin{itemize}
 \item The lifting of $\vlRel$ to callstacks is inductively defined as follows: 
 \begin{mathpar}
 \inferrule[Top Stack Frame]
   {}{\vlR{\st}{\vtup{\f}}{\vtup{\f}}}
 \and 
 \inferrule[Inner Stack Frame]
      {
          \vlR{\st}{\sto_1}{\sto_2}
          \and 
           \vlR{\st}{\cs_1}{\cs_2}
      }{
          \vlR{\st}{\vtup{\f, \x, \sto_1, i} \cons \cs_1}{\vtup{\f, \x, \sto_2, i} \cons \cs_2}
      }
 \end{mathpar}
  \item The liftings of $\stRel$ and $\leq$ to configurations are respectively defined as follows: 
   \begin{mathpar}
   \inferrule[$\stRel$-Configuration]
      {
          \stR{\st_1}{\st_2}
          \and
          \vlR{\st_1}{\cs_1}{\cs_2}
      }{
          \stR{\tup{\prog, \st_1, \cs_1, i}}{\tup{\prog, \st_2, \cs_2, i}}
      }
      \and
        \inferrule[$\leq$-Configuration]
      {
          \st_1 \leq \st_2
      }{
          \tup{\prog, \st_1, \cs, i} \leq \tup{\prog, \st_2, \cs, i}
      }
  \end{mathpar}  
 \end{itemize} 
\end{definition}

\begin{theorem}[Soundness]
Let $\soundnessCriterion = \tup{\frestriction, \stRel, \vlRel}$ be a soundness criterion
 for $\gstate_1 = \tup{\sset{\gstate_1}, \gval_1, \actions}$ in terms of $\gstate_2 = \tup{\sset{\gstate_2}, \gval_2, \actions}$
 and $\leq$ the pre-order induced by $\stRel$. It holds that: 
 $$ 
 \cf_1' \ssemarrow \cf_1'' \gand \cf_1 \leq \rfun{\cf_1'}{\cf_1''} \gand \stR{\cf_1}{\cf_2}
    \implies \exists \, \cf_2' \, . \, \cf_2 \ssemarrow \cf_2' \gand \stR{\rfun{\cf_1''}{\cf_1}}{\cf_2'}
 $$
\end{theorem}

\subsection{Soundness of Symbolic Analyses}

\begin{definition}[Symbolic Memory Interpretation]
Given a symbolic memory module $\smemory = \tup{\sset{\smemory}, \actions, \sea}$ 
and a concrete memory module $\cmemory = \tup{\sset{\cmemory}, \actions, \cea}$; 
an interpretation of $\smemory$ with respect to $\cmemory$ is a function 
$\interp : \sset{\smemory} \tmap (\lxs \pmap \vals) \pmap \sset{\cmemory}$ 
such that:
$$
\begin{array}{l}
\action{\smem}{\act}{\sexp, \pc}{(\smem', \sexp', \pc')} 
  \gand  \cmem = \interp(\smem, \lenv)
  \gand \seval{\pc \, \wedge \, \pc'}{\lenv} = \true \\
   \qquad \qquad \implies \exists \, \cmem' \, . \, 
     \cmem' = \interp(\smem', \lenv) 
     \gand 
     \caction{\cmem}{\act}{\seval{\sexp}{\lenv}}{(\cmem', \seval{\sexp'}{\lenv})}
\end{array}
$$
\end{definition}


\begin{definition}[Concrete-Symbolic Candidate Soundness Criterion]
 Let $\smemory = \tup{\sset{\smemory}, \actions, \sea}$ 
and $\cmemory = \tup{\sset{\cmemory}, \actions, \cea}$ be a symbolic memory and 
a concrete memory, respectively, and let $\interp : \sset{\smemory} \tmap (\lxs \pmap \vals) \pmap \sset{\cmemory}$ 
be an interpretation of $\smemory$ with respect to $\cmemory$;
the candidate soundness criterion $\soundnessCriterion(\interp) = \tup{\frestriction, \stRel, \vlRel}$ for 
$\sstateConstr(\smemory)$ in terms of $\cstateConstr(\cmemory)$ is defined as follows:  
$$
\begin{array}{lll}
\rfun{\tup{\smem_1, \ssto_1, \pc_1, \sarec_1}}{\tup{\_, \_, \pc_1', \sarec_1'}} & \semeq  & \tup{\smem_1, \ssto_1, \pc_1 \gand \pc_1', \sarec_1 \allocdown \sarec_1'}  \\ 
\stR{\sst}{\st} & \semeq & \exists \, \lenv \, . \, (\st, \lenv) \in \modls(\sst) \\
\vlR{\sst}{\sexp}{\vl} & \semeq & \exists \, \lenv \in \lenvs(\sst) \, . \, \seval{\sexp}{\lenv} = \vl
\end{array}
$$
where: 
$$
\begin{array}{lll}
   \modls(\tup{\smem, \ssto, \pc, \sarec}) 
       & \semeq & 
           \left\{ (\tup{\cmem, \sto, \arec}, \lenv) \mid
                   \seval{\pc}{\lenv} = \true \gand
                   \cmem = \interp(\smem, \lenv) \gand 
                   \sto = \seval{\ssto}{\lenv} \gand  
                   \arec = \allocint(\sarec, \lenv)  
            \right\} \\[3pt]
  \lenvs(\tup{\_, \_, \pc, \_}) 
     &\semeq & \left\{ \lenv \mid \seval{\pc}{\lenv} = \true \right\}
\end{array}
$$
\end{definition}

\begin{theorem}[Concrete-Symbolic Soundness Criterion]
Let $\interp$ be an interpretation of a symbolic memory module  $\smemory$  in terms of 
a concrete memory module $\cmemory$; then, $\soundnessCriterion(\interp) = \tup{\frestriction, \stRel, \vlRel}$ 
is a soundness criterion for $\sstateConstr(\smemory)$ in terms of $\cstateConstr(\cmemory)$.
%Let $\interp : \sset{\smemory} \tmap (\lxs \pmap \vals) \pmap \sset{\cmemory}$ be an interpretation 
%of a symbolic memory module  $\smemory = \tup{\sset{\smemory}, \actions, \sea}$  in terms of 
%a concrete memory module $\cmemory = \tup{\sset{\cmemory}, \actions, \cea}$; then, 
%$\soundnessCriterion(\interp) = \tup{\frestriction, \stRel, \vlRel}$ is a soundness criterion 
%for $\sstateConstr(\smemory)$ in terms of $\cstateConstr(\cmemory)$.
\end{theorem}

\subsection{\while: Sound Symbolic Analysis}

\begin{definition}[\while: Memory Interpretation Candidate]
The interpretation of \while memories, $\winterp : $ is inductively defined as follows: 
\begin{mathpar}
\inferrule[Empty]{}{\winterp(\emptymem, \lenv) \semeq \emptymem} 
\and 
\inferrule[Cell]
   {
     \loc = \seval{\sexp}{\lenv} 
     \and
     \vl = \seval{\sexp'}{\lenv}
   }{\winterp(\wcell{\sexp}{\prop}{\sexp'}, \lenv) \semeq \wcell{\loc}{\prop}{\vl}} 
 \and 
\inferrule[Union]
   {
     \cmem_1 = \winterp(\smem_1, \lenv) 
     \and
     \cmem_2 = \winterp(\smem_2, \lenv)
   }{\winterp(\smem_1 \dunion \smem_2, \lenv) \semeq  \cmem_1 \dunion \cmem_2}  
\end{mathpar}
\end{definition}

\begin{lemma}[\while: Memory Interpretation]
$\winterp$ is a symbolic interpretation of $\wsmems$ with respect to 
$\wcmems$. 
\end{lemma}



%   
%   \item $\kwT{store} : \sset{\gstate} \tmap \sset{\gstate}$ 
%            \hfill (\emph{notation:} $\kwT{store}(\st) \equiv \st.\kwT{store}$) 
%   %
%   %
%   \item $\kwT{ea} : \actions \tmap \sset{\gstate} \tmap \gval \pmap \power{\sset{\gstate} \times \gval}$ 
%            \hfill (\emph{notation:} $(\st', \vl') \in \kwT{ea}(\act, \st, \vl) \equiv \action{\st}{\act}{v}{(\st', v')}$) 


==> sections/sem_martin2.tex <==
%!TEX root = ../main.tex
\section{Parametric Symbolic Execution}
\label{sec:sem}

\subsection{\gil Syntax and Semantics}

\gil (pronounced \textipa{/\t{dZ}il/}) is a simple goto language with top-level procedures. It is parametric on a set of actions, $\actions$, which provide a general mechanism for interacting with \gil states. This parametricity allows us to maintain \gil states opaque throughout the meta-theoretical development and to provide parametric soundness results, minimising the burden of proof for users of \gillian.

%A \gil program can be viewed as a set of top-level procedures with distinct names.
%Every \gil program is parameterised by a set $\actions$ of actions for acting on a given \gil state. 
%

%\myparagraph{Syntax} The syntax of \gil is given below. 
%
\smallskip
\begin{display}{The Syntax of \gil}
\hspace*{-0.15cm}
\begin{tabular}{l@{\quad}l}
   $\vl \in \vals \defeq \num \in \nums \mid i \in \ints \mid \str \in \strs \mid \bool \in \bools \mid \varsigma \in \locs \mid \type \in \types \mid \fid \in \fids \mid \lst{\vl}$
   & 
   $\e \in \exprs \defeq \vl \mid \x \in \xs \mid \unop{\e} \mid \binop{\e_1}{\e_2}$
   %  \lx  \in \lxs
   \\[3pt]
   % 
    $\cm \in \cmds{\actions}$ $\defeq$ $\x := \e \mid \ifgoto{\e}{i} \mid \x := \e(\e') 
                                     \mid \x := \act(\e) \mid$ &    $\proc \in \procs{\actions}$ $\defeq$ $\procedure{f}{\x}{\lst{\cm}}$
 \vspace*{3pt}
    %
    \\
    \hspace*{1.28cm}$\x := \symb{j} \mid \x := \fresh{j} \mid \return{\e} \mid  \fail{e} \mid \vanish $
    & 
    $\prog \in \progs{\actions}$ $:$ $\fids \pmap \procs{\actions}$
 \end{tabular}
\end{display}
\smallskip

%
\gil \emph{values}, $\vl \in \vals$, include numbers, integers, strings, booleans,   symbols, types, procedure identifiers, and lists of values. Since we mainly use symbols to denote locations, we also use $\loc$ to range over the symbols throughout the paper.
\gil~\emph{expressions}, $\e \in \exprs$, include values, program variables $\x$, and various unary and binary operators. %Symbolic variables 

\gil \emph{commands} include, first of all, the standard variable assignment, conditional goto, and dynamic procedure call.\footnote{The procedure call is dynamic in that the  identifier is obtained by evaluating the caller expression. Also, to avoid clutter, we assume in the meta-theory a single parameter for all procedures. In the implementation, we allow for multiple parameters.}
Next, we have three \gil-specific commands: action execution, 
$\x := \act(\e)$, executes the action $\act \in \actions$ with the argument obtained by evaluating $\e$; and two allocations, $\x := \symb{j}$ and $\x := \fresh{j}$, which generate fresh uninterpreted and interpreted symbols, respectively. Note that $\kwT{symb}$ and $\kwT{fresh}$ are annotated with a jointly unique identifier $j$, used by the semantics. Finally, we have three additional control-flow related commands: $\kwT{return}$ terminates the execution of 
the current procedure; $\kwT{fail}$ terminates the execution of the entire program with an error; 
and $\vanish$ silently terminates the execution of the entire program without generating a result. 

%The variable assignment, goto, return, fail, and vanish commands are straightforward. 
%The procedure call is dynamic: the procedure identifier is obtained by evaluating the caller expression.
%The commands $\kwT{fresh}$ and $\kwT{symb}$ are annotated with a unique identifier $j$ to be used 
%by the semantics. 
%Finally, the action command $\x := \act(\e)$ executes the action $\act \in \actions$ on the current state with the argument resulting from the evaluation of $\e$. 

A \gil procedure, $\proc \in \procs{\actions}$ is of the form $\procedure{f}{\x}{\lst{\cm}}$, where $\f$ is its identifier, $\x$ is its formal parameter, 
and its body $\lst{\cm}$ is a sequence of \gil commands. 
%In order not to clutter the formalism, we assume that procedures have a single parameter. 
%In the implementation, however, procedures are allowed to have multiple parameters. 
%
A \gil program, $\prog \in \progs{\actions}$, is a finite partial function mapping procedure identifiers 
to their corresponding procedures. 

\myparagraph{Semantics} 
The semantics of \gil is parameterised by a state model, $\gstate \in \gstates$, defined as follows. 

%A state module describes: 
%\etag{1} the set of states on which \gil programs will operate, $\sset{\gstate}$;  
%\etag{2} the set of values stored in those states, $\gval$; and 
%\etag{3} the set of actions that can be performed on those states, $\actions$. 
%Observe, however, that one can always instantiate the semantics of \gil with a state module 
%whose actions are all deterministic, obtaining a deterministic semantics. 

\begin{definition}[State Model]\label{def:state:module}
A state model $\gstate \in \gstates$ is a triple $\tup{\sset{\gstate}, \gval, \actions}$, consisting of: 
\etag{1} a set of states on which \gil programs operate, $\sset{\gstate}$, \etag{2} a set of values stored in those states, $\gval$, and \etag{3} a set of 
actions that can be performed on those states, $\actions$. A state model defines the following functions for acting on states ($\equiv_{pp}$ denotes pretty-printing for readability): 

\begin{itemize}
   \item $\kwT{setVar} : \sset{\gstate} \tmap \xs \tmap \gval \tmap \sset{\gstate}$ 
            \hfill ($\kwT{setVar}(\st, \x, \vl) \equiv_{pp} \st.\kwT{setVar}(\x, \vl)$) 
   %
   \item $\kwT{setStore} : \sset{\gstate} \tmap (\xs \pmap \gval) \tmap \sset{\gstate}$ 
            \hfill ($\kwT{setStore}(\st, \sto) \equiv_{pp} \st.\kwT{setStore}(\sto)$) 
   %
   \item $\kwT{store} : \sset{\gstate} \tmap (\xs \pmap \gval)$ 
            \hfill ($\kwT{store}(\st) \equiv_{pp} \st.\kwT{store}$) 
   %
   \item $\kwT{ee} : \sset{\gstate} \tmap \exprs \pmap \gval$ 
            \hfill ($\kwT{ee}(\st, \e) \equiv_{pp} \st.\kwT{ee}(\e)$) 
   %
   \item $\kwT{ea} : \actions \tmap \sset{\gstate} \tmap \gval \pmap \power{\sset{\gstate} \times \gval}$ 
            \hfill ($(\st', \vl') \in \kwT{ea}(\act, \st, \vl) \equiv_{pp} \action{\st}{\act}{v}{(\st', v')}$) 
\end{itemize}
\end{definition}

The first four functions are required for interacting with the variable store, which is kept as part of the state. In particular: \etag{1} $\kwT{setVar}(\st, \x, \vl)$  sets $\x$ to $\vl$ in the store of $\st$;
\etag{2} $\kwT{setStore}(\st, \x, \sto)$ replaces the store of $\st$ with $\sto$; 
\etag{3} $\kwT{store}(\st)$ obtains the store of $\st$; and 
\etag{4} $\kwT{ee}(\st, \e)$ evaluates the expression $\e$ in the store of $\st$.
Finally, $\kwT{ea}(\act, \st, \gv)$ executes the action $\act$ on the state $\st$
with argument~$\gv$. Actions result in sets of state-value pairs, making the \gil semantics potentially non-deterministic. 

%As the variable store is kept as part of the state, \gil state modules are expected to define 
%the following functions for interacting with the variable store: 
 
%\polish{Why did we put the store inside the state?}
A state model $\gstate =  \tup{\sset{\gstate}, \gval, \actions}$ is said to be \emph{proper} 
\emph{iff} it defines the following three distinguished actions: $\kwT{assume}$,
 $\kwT{symb}$, and $\kwT{fresh}$. Onward, we assume to work with proper state models. % and  $\kwT{symb}$: that is, $\set{\kwT{assume}, \kwT{fresh}, \kwT{symb}} \subseteq A$).

%Finally, Definition~\ref{def:state:module} formalises the notion of state module. 

\begin{figure}[!t]
{\footnotesize
\begin{mathpar}
\inferrule[\textsc{Assignment}]
  {
    \cmd(\prog, \cs, i) = \x := \e
    \and
    \ee{\st}{\e} = v
    %\\\\
    %\actionT{\st}{setVar}{\x, v}{\st'}
  }{\semtrans{\st, \cs, i}{\st.\kwT{setVar}(\x, v), \cs, i{+}1}{}{\prog}{}}  	 
 %
 \and
 %
\inferrule[\textsc{Action}]
  {
    \cmd(\prog, \cs, i) = \x := \act(\e)
    \quad
    \ee{\st}{\e} = v
    \quad
     \action{\st}{\act}{v}{(\st', v')}
     %\and
    %\actionT{\st'}{setVar}{\x, v'}{\st''}
  }{\semtrans{\st, \cs, i}{\st'.\kwT{setVar}(\x, v'), \cs, i{+}1}{}{\prog}{}}  	 
\\
%
\inferrule[\textsc{IfGoto - True}]
  {
    \cmd(\prog, \cs, i) = \ifgoto{\e}{j}
    \\\\
    \ee{\st}{\e} = v
    \\\\
    \actionT{\st}{assume}{v}{\st'}
  }{\semtrans{\st, \cs, i}{\st', \cs, j}{}{\prog}{}}  	 
%
\and
%
\inferrule[\textsc{IfGoto - False}]
  {
    \cmd(\prog, \cs, i) = \ifgoto{\e}{j}
    \\\\
    \ee{\st}{\lnot\e} = v
    \\\\
    \actionT{\st}{assume}{v}{\st'}
  }{\semtrans{\st, \cs, i}{\st', \cs, i+1}{}{\prog}{}}  	 
%
\and
\vspace*{-0.1cm}
\inferrule[\textsc{Symb}]
  {
      \cmd(\prog, \cs, i) = \x := \symb{j}
      \\\\ 
      \actionT{\st}{fresh}{j}{(\st', v')}
  }{
    \semtrans{\st, \cs, i}{\st'.\kwT{setVar}(\x, v'), \cs, i{+}1}{}{\prog}{}
  }
 %
 \and 
 %
 \inferrule[\textsc{Fresh}]
  {
     \cmd(\prog, \cs, i) = \x := \fresh{j}
      \\\\ 
    \actionT{\st}{symb}{j}{(\st', v')}
  }{
    \semtrans{\st, \cs, i}{\st'.\kwT{setVar}(\x, v'), \cs, i{+}1}{}{\prog}{}
  }
  \and
%
\inferrule[\textsc{Call}]
  {
    \cmd(\prog, \cs, i) = \e(\e')
    \\\\
    \ee{\st}{\e} = \f
    \and
    \ee{\st}{\e'} = v
    \\\\
    \cs' = \vtup{\f, \x, \st.\kwT{store}, i+1} \cons \cs
    %\quad
    %\actionT{\st}{setStore}{\bconf{\f.\kwT{arg} \mapsto v}}{\st'}
  }{\semtrans{\st, \cs, i}{\st.\kwT{setStore}(\btup{\f.\kwT{arg} \mapsto v}), \cs', 0}{}{\prog}{}}  	
%
\and
%
\inferrule[\textsc{Return}]
  {
     \cmd(\prog, \cs, i) = \return{\e}
      \and
    \ee{\st}{\e} = v   
     \\\\
    \cs = \vtup{-, \x, \sto, j} \cons \cs'
    \and 
    \st' = \st.\kwT{setStore}(\sto)
  }{
    \semtrans{\st, \cs, i}{\st'.\kwT{setVar}(\x, v'), \cs', j}{}{\prog}{}
  }
  \qquad
  %
 \inferrule[\textsc{Top Return}]
  {
     \cmd(\prog, \cs, i) = \return{\e}
      \\\\
    \ee{\st}{e} = v
  }{
    \semtrans{\st, \vtup{\fid}, i}{\st, \vtup{\fid}, i}{}{\prog}{\normal{v}}
  } 
  %
  \qquad
  %
 \inferrule[\textsc{Fail}]
  {
     \cmd(\prog, \cs, i) = \fail{e}
      \\\\
    \ee{\st}{\e} = \vl
  }{
    \semtrans{\st, \cs, i}{\st, \cs, i}{}{\prog}{\error{\vl}}
  } 
\end{mathpar}}
%
\vspace*{-0.35cm}
\caption{Semantics of \gil: $\fullsemtrans{\st, \cs, i}{\st', \cs', j}{}{\prog}{\outcome'}{\outcome}$}
\label{fig:sem}
\vspace{-0.5cm}
%
\end{figure}

\smallskip
\begin{display}{\gil Semantic Domains for $\gstate =  \tup{\sset{\gstate}, \gval, \actions}$}
\begin{tabular}{lr@{\ \ }c@{\ \ }l@{\quad}l}
   %
   Call stacks: & $\cs \in \css{\gstate} $ & $\defeq$ & $ \vtup{\f} \mid \vtup{\f, \x, \sto, i} \cons \cs$ & where: $\f \in \fids$, $\x \in \xs$, $\sto : \xs \pmap \gval$, $i \in \ints$\\
   %
   Configurations: & $\cf \in \cfs{\gstate}$    & $\defeq$ & $\tup{\prog, \st, \cs, i}$     & where: $\prog \in \progs{\actions}$, $\st \in \sset{\gstate}$, $\cs \in \css{\gstate}$, $i \in \ints$ \\
   % 
   Outcomes: & $\outcome \in \outcomes$  & $\defeq$ &  $\cont \mid \normal{v} \mid \error{v}$ & where: $v \in \gval$
 \end{tabular}
\end{display}
\smallskip

The semantics of \gil is defined in Figure~\ref{fig:sem} in small-step style, meaning that it keeps track of the execution 
context of the calling procedure every time a new procedure is called, so that it
knows where to return the control when the execution of the called procedure is finished. 
We achieve this by using call stacks~\cite{.}.
A \emph{call stack} $\cs \in \css{\gstate}$ is a \emph{non-empty} list of stack frames. 
A top level stack frame~$\vtup{\f}$ consists solely of the identifier of the procedure which started the 
execution. 
An inner stack frame~$\vtup{\f, \x, \sto, i}$ is composed of: 
\etag{1}~the identifier $\f$ of the procedure being executed;
\etag{2}~the variable $\x$ to which the return value of $\f$ will be assigned; 
\etag{3}~the store $\sto$ of the caller of $\f$; and 
\etag{4}~the index $i$ to which the control is transferred when the execution of $\f$ terminates.
 
Additionally, to capture the flow of the execution, we use outcomes, $\outcome \in \outcomes$. \gil has three possible outcomes: 
\etag{1} the continuation outcome, $\cont$, signifying that the execution should 
proceed; 
\etag{2} the return outcome $\normal{\gvl}$, signifying that there was a top level return with value $\gvl$; 
and 
\etag{3} the error outcome $\error{\gvl}$, signifying that the execution \emph{failed} with value $\gvl$. In the rules, if the outcome is elided, it is to be interpreted as the continuation outcome. Intuitively, 
a semantic transition can only occur when the outcome of the previous command is the continuation outcome. 

Semantic transitions for \gil commands have the form $\fullsemtrans{\st, \cs, i}{\st', \cs', j}{\gstate}{\prog}{\outcome'}{\outcome}$, 
meaning that, given a \gil program $\prog$, and starting from the state~$\st$ and outcome $\outcome$, the evaluation of 
the $i$-th command of the leading procedure of the call stack $\cs$ generates the state~$\st'$, call stack~$\cs'$, and outcome $\outcome'$, and the next command to be evaluated, if applicable, is the $j$-th command of the leading procedure of $\cs'$.
 
%The rules are given in Figure~\ref{fig:sem}. 


\begin{wrapfigure}{R}{0.44\textwidth}
\begin{minted}[fontsize=\scriptsize]{ocaml}
module type State = sig 
    type t  (** Type of states  *)
    type vt (** Type of values  *)
    type a  (** Type of actions *)

    val init     : t 
    val setVar   : t -> Var -> vt -> t 
    val setStore : t -> (Var, vt) Map -> t 
    val store    : t -> (Var, vt) Map 
    val ee       : t -> Expr.t -> vt 
    val ea       : a -> t -> vt -> (t * vt) list 
    val assume   : t -> vt -> (t * vt) list 
    val symb     : t -> vt -> (t * vt) list   
    val fresh    : t -> vt -> (t * vt) list 
end

module type Allocator = sig 
    type t    (** Type of allocators            *)
    type vtus (** Type of uninterpreted symbols *)
    type vtis (** Type of interpreted symbols   *)

    val alloc : t -> int -> bool -> (t * vt)
end
\end{minted}
\vspace*{-0.35cm}
\caption{OCaml State Signature}\label{fig:ocaml:state:sig}
\vspace{-0.9cm}
\end{wrapfigure}

\myparagraph{Implementation}
The \gil semantics is implemented as an OCaml functor parameterised by an 
OCaml module with type \texttt{State}, as given in Figure~\ref{fig:ocaml:state:sig}. 
The \texttt{State} module type precisely follows our formal definition of state 
models as in Definition~\ref{def:state:module}. 
Furthermore, the code of the \gil interpreter also follows the formal definition 
of the semantics given in Figure~\ref{fig:sem}. 


\subsubsection{\gil Allocation}

%
Fresh value generation is a common source of technical clutter that is often 
omitted or hand-waved in the formal presentation of program analyses.
%
\gillian relieves the user of the framework 
from needing to reason about this issue by
having built-in fresh-value \emph{allocators}~\cite{.}.

\begin{definition}[Allocator Model]
\label{def:am}
An allocator model $\allocator \in \allocators$
  \mbinline{In the definition \(\allocators\), reduce the kerning between the \(\mathcal{A}\) and the \(L\),
    or use a \(\mathcal{L}\) instead of \(L\): it still looks some kind of application to me as-is.}
is a pair $\tup{\sset{\allocator}, \gval}$ consisting of: 
\etag{1} a set $\sset{\allocator} \ni \arec$ of allocators; and 
\etag{2} a set $\gval$ of values to allocate.
It exposes the following function:

\smallskip
$\allocf : \sset{\allocator} \tmap \ints \tmap \power{\gval} \pmap \sset{\allocator} \times \gval \qquad\quad 
$
\smallskip
 
\noindent 
which satisfies the well-formedness constraint: 

\smallskip
$(\arec', \gvl) = \allocf(\arec, j, Y) \implies \gvl \in Y$.
\end{definition}

%\smallskip
%and is pretty printed $((\arec', \gvl) = \allocf(\arec, j, Y) \equiv_{pp} \alloc{\arec}{j}{\arec', \gvl}{Y})$

Informally, $\allocf(\arec, j, Y)$ generates a fresh value~$v$ taken from 
$Y \subseteq \gval$, associates it with the \emph{allocation site}\footnote{An allocation site $j$ is the program point that is associated with either the $\symb{j}$ or the $\fresh{j}$ command.}
\mbinline{This footnote should not be a footnote, but should be defined when defining these commands.} uniquely identified by the integer $j$, and returns it together with a new allocator. We discuss allocators and their properties in more detail in \S\ref{subsec:symb:soundness}, in the context of our soundness results.

\myparagraph{Implementation}
\mbinline{This looks like this should be placed in the artefact documentation and not in the paper.}
We implement allocator models as shown in Figure~\ref{fig:ocaml:state:sig}. As we do not have the expressive power to pass arbitrary subsets in OCaml, we instead require two separate types, $\mathtt{vtus}$ and $\mathtt{vtis}$ used generating fresh uninterpreted and interpreted symbols, respectively, as regulated by the additional boolean flag passed to the $\allocf$ function. Alternatively, we could have opted for two separate allocators, but have judged that this would introduce more clutter into the code. We show how allocators can be used in practice in \S\ref{sec:concverssym}.



\subsection{\while: Actions and Compilation to \gil}\label{subsec:while:compiler}

In order to compile \while to \gil, we first pick a set of actions $\actionswhile$ for acting on \while states. We have four operations on objects---allocation, lookup, mutation, and disposal---and assigning an action to each of those would be a reasonable first attempt. However, since \gillian has a built-in allocator for 
generating fresh locations, we do not need a separate action for object allocation, arriving at the set of actions $\actionswhile = \lbrace \lookupAction, \mutateAction, \disposeAction \rbrace$. 
\mbinline{Nitpicking: the underline is not at the same depth for each of these actions. Maybe use the \texttt{ul} command instead of \texttt{underline}?}
\mbinline{More importantly, why \(\actionsZ\) is not included in this set?}

\begin{figure}
{\footnotesize
\begin{mathpar}
\inferrule[\textsc{Assignment}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\x := \e, \wpc) \semeq \\
      {\begin{array}{l}
        \wpc:  \x := \e  \\ 
         \nextpc{\wpc + 1}
       \end{array}} 
      \end{array}}
  }
%  
 \and 
 %
 \inferrule[\textsc{Skip}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wskip, \wpc) \semeq \\
      {\begin{array}{l}
        \wpc: \ifgoto{\true}{(\wpc + 1)} \\ 
         \nextpc{\wpc + 1}
       \end{array}} 
      \end{array}}
  }
 %
 \and 
 %
  \inferrule[\textsc{Return}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wreturn{\e}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \return{\e} \\  
         \nextpc{\wpc+1}
       \end{array}} 
      \end{array}}
  }
  %
 \and 
 %
   \inferrule[\textsc{Call}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\x := \fid(\e), \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \x := \fid{\e} \\  
         \nextpc{\wpc+1}
       \end{array}} 
      \end{array}}
  }
 %
 \and
 %
 \inferrule[\textsc{Sequence}]
  {
     \compWhile(\cw_1, \wpc) = (\lst{\cm}_1, \wpc_1) \\\\
     \compWhile(\cw_2, \wpc_1) = (\lst{\cm}_2, \wpc_2)
  }{
     {\begin{array}[t]{l}
      \compWhile(\cw_1; \cw_2, \wpc) \semeq \\
      {\begin{array}{l}
         \lst{\cm}_1 \\ 
         \lst{\cm}_2 \\ 
         \nextpc{\wpc_2 + 1}
       \end{array}} 
      \end{array}}
  }
%
\and 
%
  \inferrule[\textsc{If}]
  {
     \compWhile(\cw_1, \wpc+1) = (\lst{\cm}_1, \wpc_1) \\\\
     \compWhile(\cw_2, \wpc_1+1) = (\lst{\cm}_2, \wpc_2)
  }{
     {\begin{array}[t]{l}
      \compWhile(\wif{\e}{\cw_1}{\cw_2}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \ifgoto{(\gnot \, \e)}{(\wpc_1+1)} \\ 
         \lst{\cm}_1 \\ 
         \wpc_1: \ifgoto{\true}{\wpc_2} \\ 
         \lst{\cm}_2 \\ 
         \nextpc{\wpc_2}
       \end{array}} 
      \end{array}}
  }
  %
 \and 
 %
  \inferrule[\textsc{While}]
  {
     \compWhile(\cw, \wpc+1) = (\lst{\cm}, \wpc') 
  }{
     {\begin{array}[t]{l}
      \compWhile(\wwhile{\e}{\cw}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \ifgoto{(\gnot \, \e)}{(\wpc' +1)} \\ 
         \lst{\cm} \\ 
         \wpc': \ifgoto{\true}{\wpc} \\ 
         \nextpc{\wpc'+1}
       \end{array}} 
      \end{array}}
  }
%
\and 
%
\inferrule[\textsc{Assume}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wassume{\e}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \ifgoto{\e}{(\wpc + 2)} \\ 
          \wpc+1: \vanish \\
         \nextpc{\wpc + 2}
       \end{array}} 
      \end{array}}
  }
%
\and 
%
\inferrule[\textsc{Assert}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wassert{\e}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \ifgoto{\e}{(\wpc + 2)} \\ 
          \wpc+1: \fail{\e} \\
         \nextpc{\wpc + 2}
       \end{array}} 
      \end{array}}
  }
%
\and 
%
\inferrule[\textsc{New}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\x := \wobj{\prop_i: \e_i\mid_{i=1}^n}, \wpc) \semeq \\
      {\begin{array}{l}
         \wpc: \x :=  \symb{} \\ 
          \wpc+i: \_ := \mutateAction(\litlst{\x, \prop_i, \e_i}) \mid_{i=1}^n \\
         \nextpc{\wpc + n + 1}
       \end{array}} 
      \end{array}}
  }
 %
 \and 
 %
 \inferrule[\textsc{Lookup}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wlookup{\x}{\e}{\prop}, \wpc) \semeq \\
      {\begin{array}{l}
          \wpc: \x := \lookupAction(\x, \prop) \\
         \nextpc{\wpc + 1}
       \end{array}} 
      \end{array}}
  }
  %
  \and 
  %
  \inferrule[\textsc{Mutate}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wmutate{\e_1}{\prop}{\e_2}, \wpc) \semeq \\
      {\begin{array}{l}
          \wpc: \_ := \mutateAction(\litlst{\e_1, \prop, \e_2}) \\
         \nextpc{\wpc + 1}
       \end{array}} 
      \end{array}}
  }
  %
  \and 
  %
    \inferrule[\textsc{Dispose}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wdispose{\e}, \wpc) \semeq \\
      {\begin{array}{l}
          \wpc: \_ := \disposeAction(\e) \\
         \nextpc{\wpc + 1}
       \end{array}} 
      \end{array}}
  }
 \end{mathpar}}
 \vspace*{-0.35cm}
\caption{\while-to-GIL. $\compWhile : \cws \tmap \ints \tmap \litlst{\cmds{\actionswhile}} \times \ints$}
 \vspace*{-0.3cm}
\label{while:compiler}
\end{figure}
\mbinline{The notation \(\nextpc{}\) is understandable, but needs to be explicited.}

\mbinline{Why not:
\begin{mathpar}
 \inferrule[\textsc{Skip}]
  {}{
     {\begin{array}[t]{l}
      \compWhile(\wskip, \wpc) \semeq \\
      {\begin{array}{l}
         \nextpc{\wpc}
       \end{array}} 
      \end{array}}
  }
\end{mathpar}
}

\mbinline{For the compilation to work, you need the \(\_\) variable not to be used in the original \while program.}

The \while-to-\gil compiler is given in Figure~\ref{while:compiler}. It is modelled as a function 
$\compWhile : \cws \tmap \ints \tmap \litlst{\cmds{\actionswhile}} \times \ints$,
\mbinline{\(\mathcal{C}\) is used to represents both a function (the compiler) and a type (the \gil commands).}
mapping a 
\while statement $\cw \in \cws$ and a positive integer $\wpc$ (read: \emph{program counter}) 
to a sequence of \gil commands and the next available program counter. 
For instance, if $\compWhile(\cw, \wpc) = (\lst{\cm}, \wpc')$, it follows that the while 
statement $\cw$ is compiled to the sequence of \gil commands given by $\lst{\cm}$ and 
that the commands in $\lst{\cm}$ are to be labelled with indexes $\wpc$ to $\wpc'-1$. 
%meaning that $\wpc'$ is the next available index. 

The compilation rules are standard. 
For illustration purposes, we explain the \textsc{Assume} and \textsc{Assert} rules.
The assume statement, $\wassume{\e}$, compiles to a goto statement, 
($\ifgoto{\e}{(\wpc + 2)}$), which branches on the value of the expression to be assumed, followed by a silent cutting of the branch in which it does not hold by using the \gil command $\vanish$. 
The assert statement ($\wassert{\e}$) is compiled to the same goto statement that branches on $\e$, but this time, if the branch in which $\e$ does not hold is reached, the execution will terminate with an error by using the \gil command $\kwT{fail}$. 



\subsection{Concrete vs.~Symbolic States}
\label{sec:concverssym} 

\polish{Reasoning about programs can, at a high level, be separated into reasoning about the \emph{variable store} and about the the \emph{memory model} of the programming language in question.}
\mbinline{The previous sentence can be read as an overstatement for me.  Suggestion: replace “can” by “may” or “can sometimes”.  (In the case of JavaScript, the variable store is not what the reader thinks it is.)}
\gillian simplifies this process by providing built-in reasoning about the variable store, leaving to the user only to take care of the memory model. In particular, it is possible to lift a given memory to a \gil state by coupling said memory with an appropriate variable store and allocator. In this section, we illustrate this lifting for \emph{concrete} and \emph{symbolic} memories, obtaining concrete and symbolic states. 

Concrete memories store concrete values, $\vl \in \vals$. Symbolic memories store logical expressions, $\sexp \in \sexps$, generated by the grammar $\sexp \in \sexps \ \defeq \ \vl \mid \lx \in \lxs \mid \unop{\sexp} \mid \binop{\sexp_1}{\sexp_2}$, 
where $\lx$ ranges over a set of \emph{logical variables}, $\lxs$. 
The formal definitions of these two memory models are as follows.
 
%Symbolic memories differ from a concrete memories in that they store symbolic values 
%instead of concrete values $\vl \in \vals$. Symbolic values are represented in \gillian 
%as logical expression $\sexp \in \sexps$, generated by the following grammar: 
%$\sexp \in \sexps \ \defeq \ \vl \mid \lx \in \xs \mid \unop{\sexp} \mid \binop{\sexp_1}{\sexp_2}$. 


%\begin{definition}[Logical Expressions/Logical Environment/Interpretation]
%Logical expressions $\sexp \in \sexps$ are given by the following grammar: 
%$$
%\sexp \in \sexps \ \defeq \ \vl \mid \lx \in \xs \mid \unop{\sexp} \mid \binop{\sexp_1}{\sexp_2}
%$$
%A logical environment $\lenv : \lxs \pmap \vals$ is a partial mapping from logical variables 
%to \gil values. The interpretation of a logical expression $\sexp$ with respect to a logical 
%environment $\lenv$, written $\seval{\sexp}{\lenv}$ is inductively defined as follows: 
%\begin{mathpar}
%  \inferrule[\textsc{Value}]
%  {}{\seval{\vl}{\lenv} \semeq \vl}
%  \and
%    \inferrule[\textsc{LVar}]
%      {}{\seval{\lx}{\lenv} \semeq \lenv(\lx)}
%   \and 
%    \inferrule[\textsc{UnOp}]
%      {\seval{\sexp}{\lenv} = \vl}
%      {\seval{\unop{\sexp}}{\lenv} \semeq \sunop{\vl}}
%   \and
%    \inferrule[\textsc{BinOp}]
%      {
%        \seval{\sexp_1}{\lenv} = \vl_1
%        \and
%        \seval{\sexp_2}{\lenv} = \vl_2
%       }{\seval{\binop{\sexp_1}{\sexp_2}}{\lenv} \semeq \sbinop{\vl_1}{\vl_2}}
%\end{mathpar}
%\end{definition}


\begin{definition}[Concrete Memory Model]\label{def:cmem}
A concrete memory model $\cmemory \in \cmemories$ 
is a pair $\tup{\sset{\cmemory}, \actions}$,
consisting of a set of concrete memories, $\sset{\cmemory}$, and a set of actions $\actions$. 
A concrete memory model additionally defines a function $\cea$ for acting 
on memories: 
$$\cea : \actions \tmap \sset{\cmemory} \tmap \vals \pmap \sset{\cmemory} \times \vals
\qquad \qquad \qquad ({\cea}(\act, \cmem, \vl) \equiv_{pp} \cmem.\act(\vl))$$
\end{definition}
\mbinline{This is the first occurence of a usage of \(\cmem\) representing a memory.}

\begin{definition}[Symbolic Memory Model]\label{def:smem}
A symbolic memory model $\smemory \in \smemories$ 
is a pair $\tup{\sset{\smemory}, \actions}$,
consisting of a set of symbolic memories $\sset{\smemory}$ and a set of actions $\actions$. 
A symbolic memory model additionally defines a function $\sea$ for acting 
on memories: 
 $$\begin{array}{c}\sea : \actions \tmap \sset{\smemory} \tmap \sexps \tmap \pcs \pmap\power{\sset{\smemory} \times \sexps \times \pcs} \\
  ((\smem', \sexp', \pc') \in {\sea}(\act, \smem, \sexp, \pc) \equiv_{pp} \action{\smem}{\act}{\sexp, \pc}{(\smem', \sexp', \pc')})\end{array}$$
where $\pc \in \pcs \subset \sexps$, addressed shortly, is a boolean logical expression.
\end{definition}
\mbinline{It is not clear at all what is the difference between \(\pcs\) and \(\sexps\) in this definition, let alone their actual definitions.}

%\begin{definition}[Symbolic Memory Module]
%A symbolic memory module $\smemory \in \smemories$ is a triple $\tup{\sset{\smemory}, \actions, \sea}$
%consisting of: \etag{1} a set of symbolic memories $\sset{\smemory}$, \etag{2} a set of actions $\actions$, 
%and \etag{3} a function:
%
%$\sea : \actions \tmap \sset{\smemory} \tmap \sexps \tmap \pcs \pmap \power{\sset{\smemory} \times \sexps \times \pcs}$ \\
% $\phantom{xxx} \quad$ 
% 
%for acting on memories. 
%\end{definition}

%\begin{definition}[Concrete/Symbolic Memory Module]\label{def:memories}
%A concrete memory module $\cmemory \in \cmemories$ is a triple $\tup{\sset{\cmemory}, \actions, \cea}$
%consisting of: \etag{1} a set of concrete memories $\sset{\cmemory}$, \etag{2} a set of actions $\actions$, 
%and \etag{3} a function $\cea : \actions \tmap \sset{\cmemory} \tmap \vals \pmap \sset{\cmemory} \times \vals$ 
%for acting on memories. 
%\end{definition}
%
%\begin{definition}[Symbolic Memory Module]
%A symbolic memory module $\smemory \in \smemories$ is a triple $\tup{\sset{\smemory}, \actions, \sea}$
%consisting of: \etag{1} a set of symbolic memories $\sset{\smemory}$, \etag{2} a set of actions $\actions$, 
%and \etag{3} a function:
%
%$\sea : \actions \tmap \sset{\smemory} \tmap \sexps \tmap \pcs \pmap \power{\sset{\smemory} \times \sexps \times \pcs}$ \\
% $\phantom{xxx} \quad$ (\emph{notation:} $(\smem', \sexp', \pc') \in \hat{\kwT{ea}}(\act, \smem, \sexp, \pc) \equiv \action{\smem}{\act}{\sexp, \pc}{(\smem', \sexp', \pc')}$)
% 
%for acting on memories. 
%\end{definition}

Given a concrete memory, $\cmem \in \sset{\cmemory}$, we construct a concrete state $\st$ by coupling
$\cmem$ with a concrete store $\sto : \xs \pmap \vals$ and a concrete allocator $\arec \in \sset{\allocator}_{\vals}$. 
Analogously, given a symbolic memory, $\smem \in \sset{\smemory}$, we construct a symbolic state $\sst$ by 
coupling $\smem$ with a symbolic store $\ssto : \xs \pmap \sexps$ and a symbolic allocator 
$\sarec \in \sset{\allocator}_{\sexps}$. In the symbolic case, we also include in the constructed state $\sst$ a boolean expression $\pc \in \pcs$, referred to as the \emph{path condition} of $\sst$. 
Path conditions~\cite{.} bookeep the constraints on the symbolic variables that led the execution to the 
current symbolic state. 
%
The liftings from concrete and symbolic memories to the appropriate states are formally described~below. We write $\actionsZ$  to refer to the set of mandatory actions $\set{\kwT{assume}, \kwT{fresh}, \kwT{symb}}$.
\mbinline{A backward link to the definition of proper state models would be appreciated here.}

\begin{definition}[Concrete State Constructor (\cstateConstr)]\label{def:concrete:lifting}
Given an allocator $\allocator = \tup{\sset{\allocator}, \vals}$, the 
concrete state constructor $\cstateConstr : \cmemories \tmap \gstates$ is defined as  
$\cstateConstr(\tup{\sset{\cmemory}, \actions}) \semeq \tup{\sset{\gstate}, \vals, \actions  \dunion \actionsZ}$,
where: 

{\small
\begin{tabular}{lll}
   \multicolumn{3}{l}{\mybullet $\sset{\gstate} = \sset{\cmemory} \times \pfunset{\xs}{\vals} \times \sset{\allocator}_{\vals}$} \\ 
  %
  \mybullet $\kwT{setVar}(\tup{\cmem, \sto, \arec}, \x, \vl)$ 
       & $\semeq$ & 
       $\tup{\cmem, \sto[\x \mapsto \vl], \arec}$ \\ 
  %
  \mybullet $\kwT{setStore}(\tup{\cmem, \_, \arec}, \sto)$
     & $\semeq$ & 
     $\tup{\cmem, \sto, \arec}$ \\ 
  %
  \mybullet $\kwT{store}(\tup{\_, \sto, \_})$
    & $\semeq$ & 
    $\sto$ \\
  %
  \mybullet $\kwT{ee}(\tup{\_, \sto, \_}, \e)$
    & $\semeq$ & 
    $\ceval{\e}{\sto}$ \\
 %
 \mybullet $\kwT{ea}(\act, \tup{\cmem, \sto, \arec}, \vl)$
    & $\semeq$ & 
    $\lbrace (\tup{\cmem', \sto, \arec}, \vl') \mid (\cmem', \vl') = \cea(\act, \cmem, \vl) \rbrace$ \\
  %
   \mybullet $\kwT{assume}(\st, \vl)$
    & $\semeq$ & 
    $\lbrace (\st, \vl) \mid \vl = \true \rbrace$ \\
   %
    \mybullet $\kwT{fresh}(\tup{\cmem, \sto, \arec}, i)$
    & $\semeq$ &
     $\lbrace (\tup{\cmem, \sto, \arec'}, \varsigma) \mid \alloc{\arec}{i}{\arec', \varsigma}{\locs} \rbrace $ \\
    %
    \mybullet $\kwT{symb}(\tup{\cmem, \sto, \arec}, i)$
    & $\semeq$ &
     $\lbrace (\tup{\smem, \ssto, \arec'}, \vl) \mid \alloc{\arec}{i}{\arec', \vl}{\vals} \rbrace $ \\
    
%   \mybullet $\kwT{fresh/symb}(\tup{\cmem, \sto, \freeRec, \freeCnt}, i)$
%    & $\semeq$ & 
%    $\lbrace (\tup{\cmem, \sto, \freeRec, \freeCnt[i \mapsto \freeCnt(i){+}1]}, \vl) \mid \vl = \freeRec(i, \freeCnt(i)) \rbrace $ \\
%  %
%   \mybullet $\kwT{fresh}(\tup{\cmem, \sto, \freeRec, \freeCnt}, i)$
%    & $\semeq$ & 
%    $\left\{ {\begin{array}{l}
%          (\tup{\cmem, \sto, \freeRec[(i, j) \mapsto \loc], \freeCnt[i \mapsto j{+}1]}, \loc) \\ 
%           \quad \mid j = \freeCnt(i) \gand (i, j) \not\in \domain(\freeRec) \gand \loc \not\in \rng(\freeRec) 
%           \end{array}} \right\}$ \\
%  %
%   \mybullet $\kwT{symb}(\tup{\cmem, \sto, \freeRec, \freeCnt}, i)$
%    & $\semeq$ & 
%    $\left\{ {\begin{array}{l}
%          (\tup{\cmem, \sto, \freeRec[(i, j) \mapsto \vl], \freeCnt[i \mapsto j{+}1]}, \vl) \\ 
%           \quad \mid j = \freeCnt(i) \gand (i, j) \not\in \domain(\freeRec) \gand \vl \not\in \rng(\freeRec) 
%           \end{array}} \right\}$ \\
\end{tabular}}
\end{definition}


\begin{definition}[Symbolic State Constructor ($\sstateConstr$)]\label{def:symbolic:lifting}
Given an allocator $\hat\allocator = \tup{\sset{\hat\allocator}, \sexps}$, the 
symbolic state constructor $\sstateConstr : \smemories \tmap \gstates$ is defined as 
$\sstateConstr(\tup{\sset{\smemory}, \actions}) \semeq \tup{\gsstate, \sexps, \actions  \dunion \actionsZ}$,
where: 

{\small
\begin{tabular}{lll}
   \multicolumn{3}{l}{\mybullet $\gsstate = \sset{\smemory} \times \pfunset{\xs}{\sexps} \times \sset{\allocator}_{\sexps} \times \pcs$} \\ 
  %
  \mybullet $\kwT{setVar}(\tup{\smem, \ssto, \sarec, \pc}, \x, \sexp)$ 
       & $\semeq$ & 
       $\tup{\smem, \ssto[\x \mapsto \sexp], \sarec, \pc}$ \\ 
  %
  \mybullet $\kwT{setStore}(\tup{\smem, \_, \sarec, \pc}, \ssto)$
     & $\semeq$ & 
     $\tup{\smem, \ssto, \sarec, \pc}$ \\ 
  %
  \mybullet $\kwT{store}(\tup{\_, \ssto, \_, \_})$
    & $\semeq$ & 
    $\ssto$ \\
  %
  \mybullet $\kwT{ee}(\tup{\_, \ssto, \_, \_}, \e)$
    & $\semeq$ & 
    $\ssto(\e)$ \\
 %
 \mybullet $\kwT{ea}(\act, \tup{\smem, \ssto, \sarec, \pc}, \sexp)$
    & $\semeq$ & 
    $\lbrace (\tup{\smem', \ssto, \sarec, \pc \, \wedge \pc'}, \sexp') \mid (\smem', \sexp', \pc') \in \sea(\act, \smem, \sexp) \rbrace$ \\
  %
   \mybullet $\kwT{assume}(\tup{\smem, \ssto, \sarec, \pc}, \pc')$
    & $\semeq$ & 
    $\lbrace (\tup{\smem, \ssto, \sarec, \pc \gand \pc'}, \true) \mid \pc \gand \pc' \, \text{not \unsat} \rbrace$ \\%, if $\pc \gand \pc'$ \sat \\
  %
  \mybullet $\kwT{fresh}(\tup{\smem, \ssto, \sarec, \pc}, i)$
    & $\semeq$ &
    $\lbrace (\tup{\cmem, \sto, \sarec', \pc}, \varsigma) \mid \alloc{\sarec}{i}{\sarec', \varsigma}{\locs} \rbrace $ \\
      %
  \mybullet $\kwT{symb}(\tup{\smem, \ssto, \sarec, \pc}, i)$
    & $\semeq$ &
    $\lbrace (\tup{\cmem, \sto, \sarec', \pc}, \lx) \mid \alloc{\sarec}{i}{\sarec', \lx}{\lxs} \rbrace $ \\
  
 %  \mybullet $\kwT{assume}(\tup{\_, \_, \pc, \_, \_}, \pc')$
  %  & $\semeq$ & 
  %  $\lbrace \rbrace$, if $\pc \gand \pc'$ \\
  %
%   \mybullet $\kwT{fresh/symb}(\tup{\smem, \ssto, \pc, \sfreeRec, \sfreeCnt}, i)$
%    & $\semeq$ & 
%    $\lbrace (\tup{\smem, \ssto, \pc, \sfreeRec, \sfreeCnt[i \mapsto \sfreeCnt(i){+}1]}, \sexp) \mid \sexp = \sfreeRec(i, \sfreeCnt(i)) \rbrace$ \\ 
%  %
%   \mybullet $\kwT{fresh}(\tup{\smem, \ssto, \pc, \sfreeRec, \sfreeCnt}, \loc)$
%    & $\semeq$ & 
%      $\left\{ {\begin{array}{l}
%          (\tup{\smem, \ssto, \pc, \sfreeRec[(i, j) \mapsto \loc], \sfreeCnt[i \mapsto j{+}1]}, \loc) \\ 
%           \quad \mid j = \sfreeCnt(i) \gand (i, j) \not\in \domain(\sfreeRec) \gand \loc \not\in \rng(\sfreeRec) 
%           \end{array}} \right\}$ \\
%  %
%   \mybullet $\kwT{symb}(\tup{\smem, \ssto, \pc, \sfreeRec, \sfreeCnt}, \lx)$
%    & $\semeq$ & 
%     $\left\{ {\begin{array}{l}
%          (\tup{\smem, \ssto, \sfreeRec[(i, j) \mapsto \lx], \freeCnt[i \mapsto j{+}1]}, \lx) \\ 
%           \quad \mid j = \sfreeCnt(i) \gand (i, j) \not\in \domain(\sfreeRec) \gand \lx \not\in \rng(\sfreeRec) 
%           \end{array}} \right\}$ \\
\end{tabular}}
\end{definition}

The concrete/symbolic liftings construct all of the functions that a state model exposes, with the help of the action execution function of the parameter concrete/symbolic memories and the $\kwT{alloc}$ function of the parameter concrete/symbolic allocator. 
In both cases, the construction of $\kwT{setVar}$, $\kwT{setStore}$, and 
 $\kwT{store}$ is straightforward. The remaining cases are described below.
 
\myparagraph {\prooflab{EvalExpr}} %The function $\kwT{ee}$ evaluates the given expression in the store of a given state. 
In the concrete case, expression evaluation is performed concretely (we use $\ceval{\e}{\sto}$ to denote the
standard expression evaluation of $\e$ with respect to $\sto$). In the symbolic case, it amounts to substituting all the program variables in $\e$ with their associated logical 
expressions given by the store (we denote this substitution by $\ssto(\e)$).  

\myparagraph{\prooflab{Action}} Action execution amounts to calling the function $\kwT{ea}$ of the parameter memory.
% and wrapping the result with the current store and allocator (and path condition, in the symbolic case). 
Observe that symbolic actions, unlike concrete actions, may branch. For this reason, they additionally 
generate a logical expression, $\pc'$, describing the conditions under which the chosen 
branch is taken. Hence, the path condition of the obtained state is a conjunction of $\pc'$ with the path 
condition $\pc$ of the original state. 

\myparagraph{\prooflab{Assume}} The function $\kwT{assume}$ generates a set of states in which 
the given value \emph{holds}. 
In the concrete case, we return the singleton set containing the original state when given the value $\true$
 and the empty set otherwise. 
In the symbolic case, we simply conjunct the given logical expression with the current path condition and require it to not be unsatisfiable.
Note that if we can prove that the new path condition is unsatisfiable, we also generate the empty set. 

\myparagraph{\prooflab{Symb/Fresh}} The functions $\kwT{symb}$/$\kwT{fresh}$ generate symbols 
using the parameter allocator. We use the arrow parameter of the allocator to indicate the set from which to pick 
the freshly generated value: $\kwT{fresh}$ picks an uninterpreted and $\kwT{symb}$ picks an interpreted symbol. Note that, as symbolic values are logical expressions, it makes sense to pick a fresh logical variable when generating a fresh interpreted symbol and then later impose constraints on it via the $\kwT{assume}$ function.

%In the concrete state, this evaluation is done concretely (we use $\ceval{\e}{\sto}$ to denote the
%standard expression evaluation of $\e$ with respect to $\sto$). In the symbolic case, expression
%evaluation amounts to substituting all the program variables in $\e$ with their associated logical 
%expressions given by the symbolic store (we use $\ssto(\e)$ to denote that substitution).  



\begin{figure}[!t]
\begin{minipage}{0.48\textwidth}
\begin{minted}[fontsize=\scriptsize]{ocaml}
module type CMemory = sig 
    type t          (** Type of concrete memories *)
    type a          (** Type of actions           *)
    type vt = Val.t (** Type of concrete values   *)
    
    val ea : a -> t -> vt -> (t * vt) option 
end
\end{minted}
\medskip
\begin{minted}[fontsize=\scriptsize]{ocaml}
module CState
  (CMem  : CMemory) 
  (Alloc : Allocator with type vtus = Symb.t 
                      and type vtis = Val.t) : 
    (State with type a = CMem.a) = struct 
  type vt = Val.t
  type t  = CMem.t * vt Store * Alloc.t 
    ...
end 
\end{minted}
\end{minipage}
%
\begin{minipage}{0.48\textwidth}
\begin{minted}[fontsize=\scriptsize]{ocaml}
module type SMemory = sig 
    type t             (** Type of concrete memories *)
    type a             (** Type of actions           *)
    type vt = LExpr.t  (** Type of symbolic values   *)
    
    val ea : a -> t -> vt -> vt -> (t * vt * vt) list  
end
\end{minted}
\medskip
\begin{minted}[fontsize=\scriptsize]{ocaml}
module SState
  (SMem  : SMemory) 
  (Alloc : Allocator with type vtus = Symb.t
                      and type vtis = LVar.t) :
    (State with type a = SMem.a) = struct 
  type vt = LExpr.t
  type t  = SMem.t * vt Store * Alloc.t * vt   
    ...
end 
\end{minted}
\end{minipage}
\vspace*{-0.2cm}
\caption{OCaml Signatures for Concrete and Symbolic States and Memories}\label{fig:make:state}
\vspace*{-0.5cm}
\end{figure}

\myparagraph{Implementation}
The concrete and symbolic state transformers are implemented as OCaml functors,
respectively parameterised by an OCaml module with type \texttt{CMemory} and an OCaml
module with type \texttt{SMemory}, as given in Figure~\ref{fig:make:state}. 
Both functors are additionally parameterised by a module with type \texttt{Allocator}
for the generation of fresh values. % corresponding to the allocator. 
The \texttt{CMemory} and \texttt{SMemory} module types precisely follow our formal characterisation of 
concrete and symbolic state models as per Definitions~\ref{def:cmem} and~\ref{def:smem}. 
Furthermore, the functors \texttt{CState} and \texttt{SState}  also follow the concrete and symbolic 
liftings described in Definitions~\ref{def:concrete:lifting} and~\ref{def:symbolic:lifting}. 
For instance, one can check that their respective carrier types (both called \texttt{t}) 
precisely match the carrier sets of the \emph{lifted} states. 

Additionally, \gillian comes with a first-order solver, which supports reasoning about, for example, numbers, string, lists, and sets. It is used, for one, in expression evaluation, where it attempts to apply a number of algebraic identities as well as heuristics in order simplify the expression resulting from the substitution $\ssto(\e)$. We also use this solver to discharge satisfiability and entailment questions (e.g.~$\pc \vdash \sexp = \sexp'$), by encoding them into  Z3~\cite{.}. 
This makes it easy for the user of the framework to swiftly develop new memory models, 
as they only need to define the actions that interact with their memory
type, while relying on the framework for solving the first-order queries that arise from those actions.%\footnote{\polish{I 
%want to say something about Z3 and what do we actually support.}}
%The first order solver is simply a front-end to Z3~\cite{.}. 

\subsection{\while: Concrete and Symbolic Memories}

We show how to obtain a concrete/symbolic interpreter %\footnote{\polish{Should I say semantics or interpreter?}}
for \while by combining the 
\while-to-\gil compiler given in \S\ref{subsec:while:compiler} with a concrete/symbolic \while memory model. 
In practice, in order to obtain an off-the-shelf fully functional interpreter, 
the user of \gillian only needs to provide a compiler from the target language to \gil, together 
with an implementation of the appropriate memory model.  
For a concrete interpreter, they need to provide a concrete memory; \emph{mutatis mutandis} 
for a symbolic interpreter. 
\mbinline{My ablative absolute is rusty: can’t this sentence be rephrased using the word “respectively”?}
Expectedly, the actions of the memory model must match those of the syntax 
(used by the compiled code).

The first step towards defining a memory model is to pick the carrier set of the model, 
\mbinline{I don’t understand what you mean by “carrier set”.}
in this case: the set of \while memories. 
We define a concrete \while memory as a partial mapping from symbols (corresponding to object locations
\mbinline{Wait, how specific is this? I think that only in the \while language it actually corresponds to object locations. I suggest to add a “in the case of \while” in this parenthesis}) and strings 
(corresponding to property names) to values; formally: $\cmem \in \wcmems: \locs \times \strs \pmap \vals$. 
Analogously, we define a symbolic memory to be a partial mapping from 
logical expressions and strings to logical expressions; formally: $\smem \in \wsmems: \sexps \times \strs \pmap \sexps$. 
\mbinline{This is very surprising for me: are you associating abstract symbols with the path condition that held when they were created?
    A sentence conveiying the intuition is lacking there.}
Property names are not lifted to logical expressions in the symbolic case, since the \while statements
that act on object properties do not allow the property name to be resolved dynamically. 

Having chosen the symbolic and concrete carrier sets, we can now define the functions $\cea$ and~$\sea$, for acting 
on concrete and symbolic memories, respectively. 
In particular, these functions must support the actions 
$\actionswhile = \lbrace \lookupAction, \mutateAction, \disposeAction \rbrace$ 
introduced in \S\ref{subsec:while:compiler}.
The definition of the \while concrete/symbolic actions is given in Figure~\ref{fig:while:memories}
(concrete on the left and symbolic on the right), and is straightforward.
For illustrative purposes, we describe the rules \prooflab{C-Dispose} and \prooflab{S-Dispose}.

\vspace*{-0.2cm}
\begin{figure}[!h]
\begin{minipage}{0.40\textwidth}
{\small
\begin{mathpar}
%\inferrule[Concrete Memory Type]
%{}{\cmem \in \wcmems: \locs \tmap \strs \pmap \vals}
%\\
%\inferrule[Concrete Action Type]
%{}{\cea : \actionswhile \tmap \wcmems \tmap \vals \pmap \wcmems \times \vals }
%\\
\inferrule[C-Lookup]
  {\cmem = \_ \dunion \wcell{\loc}{\prop}{\vl}}
  {\action{\cmem}{\lookupAction}{\litlst{\loc, \prop}}{(\cmem, \vl)}} 
 \\
\inferrule[C-Mutate-Present]
  {
    \cmem = \cmem' \dunion \wcell{\loc}{\prop}{\_}
    \quad
    \cmem'' = \cmem' \dunion \wcell{\loc}{\prop}{\vl}
  }{\action{\cmem}{\mutateAction}{\litlst{\loc, \prop, \vl}}{(\cmem'', \vl)}} 
 \\
\inferrule[C-Mutate-Absent]
  {
    (\loc, \prop) \notin \mathrm{dom}(\cmem)
    \and
    \cmem' = \cmem \dunion \wcell{\loc}{\prop}{\vl}
  }{\action{\cmem}{\mutateAction}{\litlst{\loc, \prop, \vl}}{(\cmem', \vl)}} 
  \\
\inferrule[C-Dispose]
  {
    \memproj{\cmem}{\loc} = (\_, \cmem')
  }{\action{\cmem}{\disposeAction}{\loc}{(\cmem', \true)}} 
%\\ 
%\inferrule[C-Proj Empty]{}
%  {\memproj{\emptymem}{\loc} \ \semeq \, (\emptymem, \emptymem)}  
%\\
%\inferrule[C-Proj Cell - 1]
%  { \loc' = \loc }
%  {\memproj{(\wcell{\loc'}{\prop}{\vl})}{\loc} \ \semeq \, (\wcell{\loc}{\prop}{\vl}, \emptymem)}  
%\\ 
%\inferrule[C-Proj Cell - 2]
%  {\loc' \neq \loc}
%  {\memproj{(\wcell{\loc'}{\prop}{\vl})}{\loc} \ \semeq \, (\emptymem, \wcell{\loc'}{\prop}{\vl})}  
%\\ 
%\inferrule[C-Proj Union]
%  {
%    \memproj{\cmem_1}{\loc} = (\cmem_1', \cmem_1'') \and
%    \memproj{\cmem_2}{\loc} = (\cmem_2', \cmem_2'')
%  }{\memproj{\cmem_1 \dunion \cmem_2}{\loc} \ \semeq \, (\cmem_1' \dunion \cmem_2', \cmem_1'' \dunion \cmem_2'')}  
\end{mathpar}}
\end{minipage}
\begin{minipage}{0.59\textwidth}
{\small
\begin{mathpar}
%\inferrule[Symbolic Memory Type]
%{}{\smem \in \wsmems: \sexps \tmap \strs \pmap \sexps}
%\\
%\inferrule[Symbolic Action Type]
%{}{\sea : \actionswhile \tmap \wsmems \tmap \sexps \tmap \pcs \pmap \power{\wsmems \times \sexps}}
%\\
\inferrule[S-Lookup]
  {
     \pc \vdash \sexp = \sexp' 
     \and
     \smem = \_ \dunion \wcell{\sexp'}{\prop}{\sexp_v}
  }{\action{\smem}{\lookupAction}{\litlst{\sexp, \prop}, \pc}{\litset{(\smem, \sexp_v, \true)}}} 
 \\
\inferrule[S-Mutate-Present]
  {
  	\pc \vdash \sexp = \sexp'' 
	\quad
    \smem = \smem' \dunion \wcell{\sexp''}{\prop}{\_}
    \quad
    \smem'' = \smem' \dunion \wcell{\sexp''}{\prop}{\sexp'}
  }{\action{\smem}{\mutateAction}{\litlst{\sexp, \prop, \sexp'}, \pc}{\litset{(\smem'', \true, \true)}}} 
 \\
\inferrule[S-Mutate-Absent]
  {
  	\memproj{\smem}{\sexp, \prop, \pc} = \emptyset
	\quad
    \smem' = \smem \dunion \wcell{\sexp}{\prop}{\sexp'}
  }{\action{\smem}{\mutateAction}{\litlst{\sexp, \prop, \sexp'}, \pc}{\litset{(\smem', \true, \true)}}} 
  \\
\inferrule[S-Dispose]
  {
    \memproj{\smem}{\sexp, \pc} = (\_, \smem')
  }{\action{\smem}{\disposeAction}{\sexp, \pc}{\litset{(\smem', \true, \true)}}}
%\\ 
%\inferrule[S-Proj Empty]{}
%  {\memproj{\emptymem}{\sexp, \pc} \ \semeq \, (\emptymem, \emptymem)}  
%\\
%\inferrule[S-Proj Cell - 1]
%  { \pc \vdash \sexp = \sexp'}
%  {\memproj{(\wcell{\sexp'}{\prop}{\sexp''})}{\sexp} \ \semeq \, (\wcell{\sexp}{\prop}{\sexp''}, \emptymem)}  
%\\ 
%\inferrule[S-Proj Cell - 2]
%  { \pc \vdash \sexp \neq \sexp'}
%  {\memproj{(\wcell{\sexp'}{\prop}{\sexp''})}{\sexp} \ \semeq \, (\emptymem, \wcell{\sexp'}{\prop}{\sexp''})}  
%\\ 
%\inferrule[C-Proj Union]
%  {
%    \memproj{\smem_1}{\sexp, \pc} = (\smem_1', \smem_1'') \and
%    \memproj{\smem_2}{\sexp, \pc} = (\smem_2', \smem_2'')
%  }{\memproj{\smem_1 \dunion \smem_2}{\sexp, \pc} \ \semeq \, (\smem_1' \dunion \smem_2', \smem_1'' \dunion \smem_2'')}  
\end{mathpar}}
\end{minipage}
%\begin{mathpar}
% \inferrule[C-Projection]
% {}{
% {\begin{array}{l}
%   \memproj{\emptymem}{\loc} \ \semeq \, (\emptymem, \emptymem) \\
%   \memproj{(\wcell{\loc}{\prop}{\vl})}{\loc} \ \semeq \, (\wcell{\loc}{\prop}{\vl}, \emptymem) \\
%   \memproj{(\wcell{\loc'}{\prop}{\vl})}{\loc} \ \semeq \, (\emptymem, \wcell{\loc}{\prop}{\vl}) \text{ if } \loc' \neq \loc
% \end{array}}}
%\end{mathpar}
\vspace{-0.3cm}
\caption{\while: Concrete and Symbolic Memories}\label{fig:while:memories}\vspace{-0.3cm}
\end{figure}

\mbinline{The \(\_\) symbol means very different things in Figures~\ref{fig:while:memories} and~\ref{while:compiler}
    (one is existential, the other is universal).}

% 
\myparagraph {\prooflab{C-Dispose}} In order to dispose  of the object at location $\loc$, we make use 
of the projection operator $\memproj{(.)}{\loc}$ to split the given memory $\cmem$ into a pair  
$(\cmem'', \cmem')$, where $\cmem''$ contains the memory cells at location $\loc$ and 
$\cmem'$ contains the others. The action returns $\cmem'$ and the value $\true$. 
The value $\true$ is returned to comply with the expected type of 
$\cea$; it is not used by the compiled code. 
\mbinline{Why not returning a unit type, then?}

\myparagraph {\prooflab{S-Dispose}} Analogously to \prooflab{C-Dispose}, this rule 
 starts by splitting the symbolic memory $\smem$ into a pair 
$(\smem'', \smem')$, where $\smem''$ contains the memory cells at 
the location \emph{denoted by} $\sexp$ and $\smem'$ contains the others.
 The symbolic projection operator,  $\memproj{(.)}{\sexp, \pc}$, then uses the 
current path condition $\pc$ to determine which heap cells have the same 
location as $\sexp$. 
The action returns $\cmem'$, the value $\true$, and the path condition $\true$. 
The returned path condition indicates that the action does not branch
and that, therefore, the path condition of the corresponding state will effectively not be updated. 



%   
%   \item $\kwT{store} : \sset{\gstate} \tmap \sset{\gstate}$ 
%            \hfill (\emph{notation:} $\kwT{store}(\st) \equiv \st.\kwT{store}$) 
%   %
%   %
%   \item $\kwT{ea} : \actions \tmap \sset{\gstate} \tmap \gval \pmap \power{\sset{\gstate} \times \gval}$ 
%            \hfill (\emph{notation:} $(\st', \vl') \in \kwT{ea}(\act, \st, \vl) \equiv \action{\st}{\act}{v}{(\st', v')}$) 

